Attack-Resilient Supervisory Control of Discrete-Event Systems: A Finite-State Transducer Approach

Resilience to sensor and actuator attacks is a major concern in the supervisory control of discrete events in cyber-physical systems (CPS). In this work, we propose a new framework to design supervisors for CPS under attacks using finite-state transducers (FSTs) to model the effects of the discrete events. FSTs can capture a general class of regular-rewriting attacks in which an attacker can nondeterministically rewrite sensing/actuation events according to a given regular relation. These include common insertion, deletion, event-wise replacement, and finite-memory replay attacks. We propose new theorems and algorithms with polynomial complexity to design resilient supervisors against these attacks. We also develop an open-source tool in Python based on the results and illustrate its applicability through a case study

==> backup.tex <==
%  Determinism relates to the ``observability'' of the FST states from the input and output. If an FST is deterministic, then we   

In addition, for any regular relation, we can construct a corresponding FST~\cite{holcombe_AlgebraicAutomataTheory_1982}.
The expressiveness of FSTs does not change by allowing a sequence of input/output symbols on single transitions because they can be reduced to FSTs in Definition~\ref{def:fst} through normalization~\cite{holcombe_AlgebraicAutomataTheory_1982,mohri_WeightedAutomataAlgorithms_2009}. A nondeterministic FST is determinizable without changing its regular relation by the powerset construction for automata (i.e., by viewing a pair of input and output symbols as a single symbol)~\cite{sipser_IntroductionTheoryComputation_1996}. 
Thus, in this work, we focus on deterministic FSTs (but potentially non-deterministic in the more standard input/output view.


We consider a class of supervisors that can rewrite actuating symbols based on past sensing symbols since this ability is essential to counter regular-rewriting attacks. Mathematically, the supervisor $\supervisor$ is modeled by an implementable FST. It is more powerful than classical ones~\cite{cassandras_IntroductionDiscreteEvent_2008} that can only allow/disable symbols and is more similar to the ones used in reactive synthesis and runtime enforcement~\cite{bloem2015shield}. 
Our formulation can reduce to the classical supervisory control setup~\cite{cassandras_IntroductionDiscreteEvent_2008}, including the previous works on attack-resilient supervisory control~\cite{wakaiki_SupervisoryControlDiscreteevent_2017,su_SupervisorSynthesisThwart_2018,goes_StealthyDeceptionAttacks_2017,carvalho_DetectionMitigationClasses_2018} by choosing the corresponding forms of the FSTs $\attacker_a$ and $\attacker_s$ (discussed in~Section~\ref{rem:recover}). 

\begin{remark}
We now further explain the meaning of being a resilient supervisor.  
The FST as the resilient supervisor derived from Theorem \ref{prop:sensor attack} may not be deterministic, i.e., its execution is not unique given the input and output sequences of symbols. But it does not directly violate Definition \ref{def:controllability}. For any word of the plant within $\desired$, there exists an execution of the supervisor to allow it. For any word of the plant outside $\desired$, the supervisor always prohibits it. 

For a given choice of nondeterminism in the resilient supervisor, the plant's language may be a subset of $\desired$. If $\desired$ captures the plant's safe words, the nondeterministic supervisor can conservatively guarantee the plant's safety. Otherwise, the resilient supervisor should be deterministic to ensure any word in $\desired$ .  
\end{remark}



==> backup/Automatica_reviews/commands.tex <==
\newcommand{\nat}{\mathbb{N}}

% \newcommand{\diag}{\mathcal{I}}

\renewcommand{\subset}{\subseteq }
\renewcommand{\supset}{\supseteq}
\renewcommand{\epsilon}{\varepsilon}

\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\c}{\circ}

\newcommand{\dom}{\mathrm{Dom}}
\newcommand{\image}{\mathrm{Image}}

\newcommand{\re}{\mathrm{Re}}

\newcommand{\rr}{\mathcal{R}}
\newcommand{\id}{\mathcal{I}}

\newcommand{\attacker}{\mathcal{A}}
\newcommand{\plant}{\mathcal{P}}
\newcommand{\supervisor}{\mathcal{S}}
\newcommand{\desired}{\mathscr{K}}

\newcommand{\astate}{\mathsf{s}}
\newcommand{\astates}{\mathsf{S}}
\newcommand{\ainit}{\mathsf{s}_\mathrm{init}}
\newcommand{\atransitions}{\mathsf{Trans}}
\newcommand{\aobservations}{\mathsf{Obs}}
\newcommand{\ainput}{\mathsf{i}}
\newcommand{\ainputs}{\mathbf{I}}
\newcommand{\aoutput}{\mathsf{o}}
\newcommand{\aoutputs}{\mathbf{O}}
\newcommand{\alabeling}{\mathsf{L}}
\newcommand{\afinal}{\mathsf{S}_\mathrm{final}}

\newcommand{\reach}{\mathsf{Reach}}

\newcommand{\ltrue}{\mathrm{True}}
\newcommand{\lfalse}{\mathrm{False}}
\newcommand{\lnext}{\mathbf{X}}
\newcommand{\luntil}{\mathbf{U}}
\newcommand{\lrelease}{\mathbf{R}}
\newcommand{\lfinal}{\mathbf{F}}
\newcommand{\lglobal}{\mathbf{G}}
\newcommand{\lall}{\mathbf{A}}
\newcommand{\lexist}{\mathbf{E}}
\newcommand{\lp}{\mathbf{P}}

\newcommand{\shift}{\mathcal{S}}
\newcommand{\iseq}[1]{#1^{(\infty)}}
\newcommand{\seq}[2]{#1^{(#2)}}
\newcommand{\set}[2]{\big\{ #1 \mid #2 \big\}}
\newcommand{\abs}[1]{\vert #1 \vert}
\newcommand{\argmax}{\mathrm{argmax}}


==> backup/Automatica_submission/attack.tex <==
\section{Regular-Rewriting Attacks}
\label{sec:attack}

We consider a wide class of \emph{regular-rewriting} attacks that can nondeterministically revise (e.g., insert, delete, and replace) sensing and actuating symbols by some \emph{regular relation}. Such very general attack models also allow for capturing of sophisticated coordinated attacks that try to e.g., bypass employed intrusion detectors and/or utilize previous system executions (e.g., replay attacks). The regular-rewriting attacks generalize previous history-independent attacks studied in~\cite{wakaiki_SupervisoryControlDiscreteevent_2017,su_SupervisorSynthesisThwart_2018,goes_StealthyDeceptionAttacks_2017,carvalho_DetectionMitigationClasses_2018} and can capture new history-dependent attacks such as finite-memory replay attacks~\cite{stuxnet,stuxnet2}. 



\subsection{Modeling Attacks by FSTs}
\label{sub:examples}

We propose to model regular-rewriting attacks using deterministic (but nondeterministic-in-input) FSTs.% 
\footnote{There is no loss of generality as all FSTs are determinizable.}
The model of FSTs can be derived from the regular relations that the attacks obey. The FSTs' nondeterminism-in-input captures all the possible (maybe infinitely-many) attack behaviors under regular relations.
% \todo{here we need to say how do we get these models; this was one of the complaints from CDC reviewers}
% \todo{YW: Please check this paragraph and the one above.}
In practice, such models (i.e., relations) may be obtained by analyzing the security services and (possible) attack surfaces from the system's architecture and deployment.
In return, the resilience analysis given later in this paper can guide the improvement of security services in the deployed system.
% or the employed security-service that are taken into account. 
% Similarly, control system resilience against considered classes of attacks may guide the design and deployment of standard (i.e., cyber) security services.
% \todo{check, is it clear for controls folks?} 

\begin{example}
Let $\ainputs' \subseteq \ainputs$. The projection attack
\begin{equation} \label{eq:projection}
    \mathrm{Project}_{\ainputs'}(\ainput) = \begin{cases}
    \ainput, &\text{ if }\quad \ainput \in \ainputs' \\
    \epsilon, &\text{ otherwise,}
  \end{cases}
\end{equation}
captures the attack that results in removing all symbols that belong to $\ainputs\setminus\ainputs'$.
%
On the other hand, the (nondeterministic) deletion attack defined as
\begin{equation} \label{eq:deletion}
  \mathrm{Delete}_{\ainputs'}(\ainput) = \begin{cases}
    \ainput, &\text{ if }\quad\ainput \in \ainputs' \\
    \epsilon \text{ or } i, &\text{ otherwise,}
  \end{cases}
\end{equation}
extends the $\mathrm{Project}_{\ainputs'}$ attack as
it captures that
the attacker may (or may not) remove symbols from $\ainputs\setminus\ainputs'$; e.g., if $\ainputs' = \ainputs$ this model can be used to capture Denial-of-Service attacks~\cite{wood2002denial} over the communication network. Finally, the (nondeterministic) injection attack defined~as
\begin{equation} \label{eq:injection}
  \mathrm{Inject}_{\ainputs'}(\ainput) = (\ainputs')^* \ainput (\ainputs')^*
\end{equation}
%
captures that a finite number of symbols from $\ainputs'$ can be added before and/or after the symbols. These attacks %, studied in~\cite{} \todo{fix}
can be represented by FSTs as shown in Fig.~\ref{ex:projection}, Fig.~\ref{ex:deletion} and Fig.~\ref{ex:injection}, respectively.
\end{example}


\begin{example}
\label{ex:rep-rem}
A replacement-removal attack defined by the rule $\phi: \ainputs \rightarrow 2^{\ainputs \cup \{\epsilon\} }$ is represented by an FST as shown in Fig.~\ref{ex:replacement-removal}.
\end{example}


\begin{example}
\label{ex:ins-rem}
Let $\ainputs' \subseteq \ainputs$. An injection-removal attack nondeterministically injects or removes symbols in $\ainputs'$ from a word. This is modeled by the FST in Fig.~\ref{ex:injection-removal}.
\end{example}

\begin{example}
For systems with continuous-state dynamics, replay attacks have been modeled and studied in e.g.,~\cite{miao_cdc13, mo_procIEEE12}. On the other hand, no such models have been introduced for supervisory control. A replay attack records a prefix of a word and replaces the rest with the repetitions of the recorded prefix, with the prefix size being bounded by the finite-memory capacity (i.e., size) $N$. This relation is regular, so can be modeled by FSTs. For example, a replay attack recording a prefix of length up to $N = 2$ for any word $\ainputs=\{\ainput_1, \ainput_2\}$ can be modeled by an FST as shown in Fig.~\ref{ex:replay}. Note that the FST can be viewed as the parallel composition of two replay attacks recording prefixes of length $1$ and $2$, respectively.
\end{example}





\begin{figure*}[!t]
\centering
\subcaptionbox{Projection\label{ex:projection}}[.2\linewidth]{
\begin{tikzpicture}
  \node[state,initial,initial text=] (s) {};
  \path[->] (s) edge[loop below] node {$\ainput \vert \epsilon$ for $\ainput \in \ainputs \backslash \ainputs'$} ()
        (s) edge[loop above] node {$\ainput \vert \ainput$ for $\ainput \in \ainputs'$} ();
\end{tikzpicture}
}
\subcaptionbox{Deletion\label{ex:deletion}}[.2\linewidth]{
\begin{tikzpicture}
  \node[state,initial,initial text=] (s) {};
  \path[->] (s) edge[loop above] node {$\ainput \vert \epsilon$ for $\ainput \in \ainputs \backslash \ainputs'$} ()
        (s) edge[loop below] node {$\ainput \vert \ainput$ for $\ainput \in \ainputs$} ();
\end{tikzpicture}
}
\subcaptionbox{Injection\label{ex:injection}}[.2\linewidth]{
\begin{tikzpicture}
  \node[state,initial,initial text=] (s) {};
  \path[->] (s) edge[loop above] node {$\epsilon \vert \ainput$ for $\ainput \in \ainputs'$} ()
        (s) edge[loop below] node {$\ainput \vert \ainput$ for $\ainput \in \ainputs$} ();
\end{tikzpicture}
}
\subcaptionbox{%
Replacement-Removal\label{ex:replacement-removal}}[.22\linewidth]{
\begin{tikzpicture}
  \node[state,initial,initial text=] (s) {};
  \path[->] (s) edge[loop below] node {$\ainput \vert \phi(\ainput)$ for $\ainput \in \ainputs$} ();
\end{tikzpicture}
}
\subcaptionbox{%
Injection-Removal\label{ex:injection-removal}}[.22\linewidth]{
\begin{tikzpicture}
  \node[state, initial right, initial text=] (s) {};
  \path[->]
  (s) edge[loop left] node[above,xshift=-0.6cm] {$\ainput \vert \epsilon$ for $\ainput \in \ainputs'$} ()
  (s) edge[loop above] node {$\epsilon \vert \ainput$ for $\ainput \in \ainputs'$} ()
  (s) edge[loop below] node {$\ainput \vert \ainput$ for $\ainput \in \ainputs \backslash \ainputs'$} ();
\end{tikzpicture}
}
\hspace{15pt}
\subcaptionbox{Replay Attack\label{ex:replay}}[.42\linewidth]{
\begin{tikzpicture}
  \node[state,initial,] (s) {};
  % \node[state, above of=s, yshift=0.2cm] (s01) {};
  % \node[state, below of=s, yshift=-0.2cm] (s02) {};
  \node[state, right of=s, yshift=0.5cm, xshift=0.5cm] (s1) {};
  \node[state, right of=s, yshift=-0.5cm, xshift=0.5cm] (s2) {};
  \node[state, right of=s1, xshift=1cm] (s11) {};
  \node[state, right of=s2, xshift=1cm] (s22) {};
  \node[state, right of=s1, yshift=0.7cm, xshift=1cm] (s3) {};
  \node[state, right of=s2, yshift=-0.7cm, xshift=1cm] (s4) {};

  \path[->] (s) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1$} (s1);
  \path[->] (s) edge[bend right] node[below] {$\ainput_2 \vert \ainput_2$} (s2);
  % \path[->] (s) edge[bend left] node[left] {$\ainput_1 \vert \ainput_1$} (s01);
  % \path[->] (s) edge[bend right] node[left] {$\ainput_2 \vert \ainput_2$} (s02);
  \path[->] (s1) edge[loop above] node[above] {$\ainput_1, \ainput_2 \vert \ainput_1$} ();
  \path[->] (s2) edge[loop below] node[below] {$\ainput_1, \ainput_2 \vert \ainput_2$} ();
  \path[->] (s1) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1$} (s3);
  \path[->] (s2) edge[bend right] node[below] {$\ainput_2 \vert \ainput_2$} (s4);
  \path[->] (s1) edge node[above] {$\ainput_2 \vert \ainput_2$} (s11);
  \path[->] (s2) edge node[below] {$\ainput_1 \vert \ainput_1$} (s22);
  \path[->] (s3) edge[loop right] node[above] {$\ainput_1,\ainput_2 \vert \ainput_1$} ();
  \path[->] (s4) edge[loop right] node[below] {$\ainput_1,\ainput_2 \vert \ainput_2$} ();
  \path[->] (s11) edge[bend left] node[right] {$\ainput_1,\ainput_2 \vert \ainput_1$} (s22);
  \path[->] (s22) edge[bend left] node[left] {$\ainput_1,\ainput_2 \vert \ainput_2$} (s11);
\end{tikzpicture}
}
\caption{FST models for common attacks.\label{fig:FST_realization}}
%\vspace{-4pt}
\end{figure*}




\subsection{Composition of Regular-Rewriting Attacks}
\label{sub:composition}

Multiple regular-rewriting attacks %connected via general architectures
at (potentially) various points of the system can %usually 
be combined into a single FST model through serial and parallel compositions of FSTs. Let $\attacker = (\astates, \allowbreak \ainit, \ainputs, \aoutputs, \allowbreak \atransitions, \afinal)$ and $\attacker' = (\astates', \ainit', \ainputs', \aoutputs', \atransitions', \allowbreak \afinal')$ be two FSTs. 
We now described how serial and parallel composition can be done.
%\todo{check}

\vspace{-12pt}
\paragraph*{Serial Composition.}
The serial composition $\attacker'' = \attacker \circ \attacker'$ is derived by connecting the FSTs $\attacker$ and $\attacker'$ in series as shown in Fig.~\ref{fig:serial},  
where the input word sequentially passes $\attacker$ and $\attacker'$. Algorithmically, the series composition is derived as follows:
\begin{enumerate}[label=(\roman*)]
  \item Perform the Cartesian product of the states and transitions,
  \item Contract the transitions on which the output of the first component is identical to the input of the second component, as well as
  \item Keep transitions with $\epsilon$ output in $\attacker$ and $\epsilon$ input in $\attacker'$, while discarding the others. The transitions with $\epsilon$ output in $\attacker$ are preserved because it can be triggered without influencing $\attacker'$; similarly for the transitions with $\epsilon$ input in $\attacker'$.
\end{enumerate}
The model derived from the series composition is still an FST. The above procedure is summarized in Algorithm~\ref{alg:composition}. Since FSTs define regular relations, Algorithm~\ref{alg:composition} also provides an FST realization for the composition of regular relations.  

\begin{lemma}[\cite{holcombe_AlgebraicAutomataTheory_1982}]
For any two FSTs $\attacker_1$ and $\attacker_2$, it holds that $\rr_{\attacker_1} \circ \rr_{\attacker_2} = \rr_{\attacker_1 \circ \attacker_2}$ where $\rr$ denotes the regular relation defined by an FST.
\end{lemma}


\begin{algorithm}[!t]
\caption{Composition of FSTs}
\label{alg:composition}
\begin{algorithmic}[1]
\Require{FSTs $\attacker = (\astates, \ainit, \ainputs, \aoutputs, \atransitions, \afinal)$ and $\attacker' = (\astates', \ainit', \aoutputs, \aoutputs', \atransitions', \afinal')$}

\State{Let $\attacker'' = \attacker \circ \attacker' = (\astates \times \astates', (\ainit, \ainit'), \ainputs, \aoutputs', \emptyset, \afinal \times \afinal')$.}

\State{Add transition $((\astate_1, \astate_1'), \ainput, \aoutput', (\astate_2, \astate_2'))$ to $\attacker''$ if there exists $\aoutput \in \aoutputs$ such that $(\astate_1, \ainput, \aoutput, \astate_2) \in \atransitions$ and $(\astate_1', \aoutput, \aoutput', \astate_2') \in \atransitions'$.}

\State{Add transition $((\astate_1, \astate'), \ainput, \epsilon, (\astate_2, \astate'))$ to $\attacker''$ for any $(\astate_1, \ainput, \epsilon, \astate_2) \in \atransitions$ and any $\astate' \in \astates'$.}

\State{Add transition $((\astate, \astate_1'), \epsilon, \aoutput, (\astate, \astate_2'))$ to $\attacker''$ for any $(\astate_1', \epsilon, \aoutput, \astate_2') \in \atransitions'$ and any $\astate \in \astates$.}

\State \Return{$\attacker''$}
\end{algorithmic}
\end{algorithm}

% Below is an example of serial composition.

\begin{example}
Consider two FSTs $\attacker_1$ and $\attacker_2$ shown in Fig.~\ref{fig:trans_1} and~\ref{fig:trans_2}, where one replaces $\ainput_1$ with $\ainput_2$ and the other injects $\ainput_3$. The overall FST attack model, captured with the serial composition of the two FSTs is derived using Algorithm~\ref{alg:composition} and shown in Fig~\ref{fig:comp}. Specifically, the composition rules for $\varepsilon$-transition is give in Line 4 and 5 of Algorithm~\ref{alg:composition}. Also, it holds that $\rr_{\attacker_1 \circ \attacker_2} = \rr_{\attacker_1} \circ \rr_{\attacker_2}$.
\end{example}


\vspace{-12pt}
\paragraph*{Parallel Composition.\footnote{Note that the parallel composition of FSTs differs from the common parallel composition for automata.}}
% \todo{check footnote}
The parallel composition $\attacker'' = \attacker \, \Vert \, \attacker'$ is derived by connecting the FSTs $\attacker$ and $\attacker'$ in parallel as illustrated in Fig.~\ref{fig:parallel}, where the input word can choose to pass either $\attacker$ or $\attacker'$. Algorithmically, the parallel composition is computed as follows.
\begin{enumerate}[label=(\roman*)]
  \item Compute the union of the states, final states, and transitions.
  \item Add a new starting state with transitions $\epsilon/\epsilon$ to the initial states $\ainit$ and $\ainit'$.
\end{enumerate}
Note that the model derived from the parallel composition is still an FST.



\paragraph*{{Composition of Attacks.}}
As mentioned above, multiple (sub)attacks modeled by FSTs can
be combined into an overall FST model. This justifies our modeling from the general system architecture in Fig.~\ref{fig:diagram} to the control diagram in Fig.~\ref{fig:control}. Specifically, in Fig.~\ref{fig:diagram}, there may be coordinated attacks from multiple deployed attack vectors with different ``point-of-entries'' from the sensors, actuators, and communication networks. 
For example, on the sensor side, there may be false data injection via sensor spoofing~\cite{gps_spoof1,shepard12} together with denial-of-service (DoS) attacks on network transmissions. The overall effect of those attacks is equivalent to their serial composition as illustrated in Fig.~\ref{fig:serial}, which is represented by a single FST $\attacker_s$ in Fig.~\ref{fig:control}. 
% \todo{give in figure captions what they are -- instead of just A1 -- it's DoS + false data injection attack} 
Similarly, if there is one of several possible attacks that may be deployed at the same ``point-of-entry'' as studied in~\cite{wakaiki_SupervisoryControlDiscreteevent_2017}, the overall effect, and the corresponding FST model, is equivalent to the parallel composition of the two FSTs capturing the basic attacks, as shown in Fig.~\ref{fig:parallel}.
% \todo{in Fig 5, the general caption was effectively for frequency constrain (i.e., Fig. 5c). So, I moved it there, and returned the old FIG 5 general caption -- does that make sense?}
% \todo{check}


\begin{figure}[!t]
\centering
\subcaptionbox{{When $n$ attacks happen simultaneously (e.g., false data injection attack on sensors $\attacker_1$, denial-of-service attack on network $\attacker_2$, ...), the overall effect can be captured by the serial composition.}\label{fig:serial}}[.45\linewidth]{
\begin{tikzpicture}
 \node (a0) {};
 \node [draw, right of=a0]  (a1) {$\attacker_1$};
 \node [right of=a1]  (a2) {$\ldots$};
 \node [draw, right of=a2]  (a3) {$\attacker_n$};
 \node [right of=a3] (a4) {};
 \draw [->, >=latex] (a0) -- (a1);
 \draw [->, >=latex] (a1) -- (a2);
 \draw [->, >=latex] (a2) -- (a3);
 \draw [->, >=latex] (a3) -- (a4);
\end{tikzpicture}
}
\hspace{0.3cm}
\subcaptionbox{{When (only) one of $n$ possible attacks may occur at a ``point-of-entry'' (i.e., attack point), the overall effect can be captured by the parallel composition of the attack models.}\label{fig:parallel}}[.45\linewidth]{
\begin{tikzpicture}
 \node (a0) {};
 \node [right of=a0]  (a2) {$\ldots$};
 \node [draw, above of=a2, yshift=-0.4cm]  (a1) {$\attacker_1$};
 \node [draw, below of=a2, yshift=0.4cm]  (a3) {$\attacker_n$};
 \node [right of=a2] (a4) {};
 \draw [->, >=latex, dashed] (a0.center) -- (a2);
 \draw [->, >=latex, dashed] (a2) -- (a4.center);
 \draw [->, >=latex] (a0.center) |- (a1);
 \draw [->, >=latex] (a1) -| (a4.center);
 \draw [->, >=latex, dashed] (a0.center) |- (a3);
 \draw [->, >=latex, dashed] (a3) -| (a4.center);
\end{tikzpicture}
}

\par\bigskip
\subcaptionbox{Modeling frequency constraints\label{fig:frequency}; e.g., the operational constraint that an FST-based attacker $\attacker$ happens once every three steps can be captured by augmenting the FST model}[.8\linewidth]{
\begin{tikzpicture}
  \node[initial, state, initial text=] (0) {};

  \node[state,right of=0,xshift=0.5cm] (1) {};
  \node[state,right of=1,xshift=0.5cm] (2) {};

  \node[draw,below of=1, xshift = -0.5cm] (3) {$\attacker'$};
  \node[draw,below of=1, xshift = 0.5cm] (4) {$\attacker'$};
  \node[draw,above of=1] (5) {$\attacker$};

  \path[->,dotted] (0) edge[bend right] node {D} (1);
  \path[->,dotted] (1) edge[bend right] node {D} (2);
  \path[->,dotted] (2) edge[bend right=35] node {E} (0);

  \path[->] (2) edge[bend right] (5);
  \path[->] (5) edge[bend right] (0);
  \path[->] (0) edge[bend right] (3);
  \path[->] (3) edge[bend left] (1);
  \path[->] (1) edge[bend left] (4);
  \path[->] (4) edge[bend right] (2);

\end{tikzpicture}
}
\caption{Modeling attack composition and attack constraint.\label{fig:fst_compose}}
\end{figure}


\begin{figure}[!t]
\centering
\subcaptionbox{FST $\attacker_1$ \label{fig:trans_1}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state, initial, initial text=] (0) {$0$};
  \node[state, right of=0] (1) {$1$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1 \vert \ainput_2$} (1);
  \path[->] (1) edge[loop right] node[right] {$\ainput_1 \vert \epsilon$} (1);
\end{tikzpicture}
}
\subcaptionbox{FST $\attacker_2$\label{fig:trans_2}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state, initial, initial text=] (0) {$0$};
  \node[state, right of=0] (1) {$1$};
  \path[->] (0) edge[bend left] node[above] {$\epsilon \vert \ainput_3$} (1);
  \path[->] (0) edge[bend right] node[below] {$\ainput_2 \vert \ainput_1$} (1);
\end{tikzpicture}
}


\par\bigskip
\subcaptionbox{Serial composition $\attacker_1 \circ \attacker_2$\label{fig:comp}}[.5\linewidth]{
\begin{tikzpicture}
  \node[state, initial, initial text=] (0) {$00$};
  \node[state, right of=0, node distance=1.5cm] (1) {$10$};
  \node[state, below of=0, node distance=1.5cm] (2) {$01$};
  \node[state, right of=2, node distance=1.5cm] (3) {$11$};

  \path[->] (0) edge node {$\ainput_1 \vert \ainput_1$} (3);
  \path[->] (1) edge[loop right] node[right] {$\ainput_1 \vert \epsilon$} (1);
  \path[->] (3) edge[loop right] node[right] {$\ainput_1 \vert \epsilon$} (3);
  \path[->] (0) edge[bend right] node[left] {$\epsilon \vert \ainput_3$} (2);
  \path[->] (1) edge[bend left] node[right] {$\epsilon \vert \ainput_3$} (3);
\end{tikzpicture}
}
\caption{Example for the composition of FSTs.\label{fig:composition}}
\end{figure}



\subsection{Imposing Constraints on Attackers}
\label{sub:constraints}

FSTs also facilitate imposing (operational) constraints and transform history-independent attacks (e.g., injection attacks from~\eqref{eq:injection}) to history-dependent attacks. 
For example, in some networked control systems, cryptographic primitives (e.g., Message Authentication Codes) can only be intermittently used due to resource constraints, and thus can only intermittently prevent injection attacks~\cite{jovanov_tac19,lesi_tecs17,lesi_tcps20}. FSTs can facilitate modeling such constraints as frequency constraints on the attacker as studied in~\cite{su_SupervisorSynthesisThwart_2018}.



\begin{example}
The FST model in Fig.~\ref{fig:frequency} shows an attacker that can perform once every three steps the attack modeled by FST $\attacker$, where $\attacker'$ is an automaton derived from $\attacker$ by removing the output symbols. Namely, $\attacker'$ accepts the same input language as $\attacker$ but does not rewrite. Actually, the states in Fig.~\ref{fig:frequency} together with the transitions drawn in dotted lines is a frequency counter with the symbols D/E representing disabling/enabling. The overall FST is built by combining the frequency counter with $\attacker$ and $\attacker'$.
\end{example}






==> backup/Automatica_submission/backup.tex <==


    


Since designing a resilient supervisor is not always possible, we consider a related problem of designing a weakly-resilient supervisor that achieves the minimal super-language of the desired language $\desired$.


\begin{definition}
\label{def:weak supervisor}
The FST $\supervisor$ is a weakly-resilient supervisor for a desired language $\desired$ iff
\begin{itemize}
  \item $\desired \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a, \attacker_s)$, and
  \item for any $\supervisor'$ that satisfies 
  $\desired \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor', \attacker_a, \attacker_s)$, it holds that 
  $L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a, \attacker_s) \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor', \attacker_a, \attacker_s)$.
\end{itemize}
\end{definition}


Generally, designing weakly-resilient supervisors is possible. And designing a resilient supervisor is possible iff the weakly-resilient supervisor is resilient (see Section~\ref{sec:design} for details). 


==> backup/Automatica_submission/bio.tex <==
% !TEX root = tac19.tex

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{yw_small.jpg}}]{Yu Wang}
% is currently a Postdoctoral Associate in the Department of Electrical and Computer Engineering at Duke University. He received his Ph.D. degree in Mechanical Engineering and his M.S. degrees in Statistics, Mathematics, and Mechanical Engineering in 2018, 2017, 2016 and 2014, respectively from the University of Illinois at Urbana-Champaign. Before that, he received his B.S. degree in Engineering Mechanics from the School of Aerospace of Tsinghua University in 2012.
% \end{IEEEbiography}


% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{alper.png}}]
% {Alper Kamil Bozkurt} received the B.S. and M.S. degrees in computer engineering from Bogazici University, Turkey, in 2015 and 2018, respectively. He is currently a Ph.D. student in the Department of Computer Science at Duke University. His research interests lie at the intersection of machine learning, control theory, and formal methods. In particular, he focuses on developing learning based algorithms that synthesize provably safe and reliable controllers for cyber-physical systems.


% \end{IEEEbiography}



% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pajic.jpg}}]{Miroslav Pajic}
%  (S'06-M'13-SM'19) received the Dipl. Ing. and M.S. degrees in electrical engineering from the University of Belgrade, Serbia, in 2003 and 2007, respectively, and the M.S. and Ph.D. degrees in electrical engineering from the University of Pennsylvania, Philadelphia, in 2010 and 2012, respectively.

% He is currently the Nortel Networks Assistant Professor in the Department of Electrical and Computer Engineering at Duke University. He also holds a secondary appointment in the Computer Science Department. His research interests focus on the design and analysis of cyber-physical systems, and in particular security-aware distributed/networked control systems, embedded systems, and high-confidence control systems.

% Dr. Pajic received various awards including the ACM SIGBED Early-Career Award, IEEE TCCPS Early-Career Award, NSF CAREER Award, ONR Young Investigator Program Award, ACM SIGBED Frank Anger Memorial Award, Joseph and Rosaline Wolf Best Dissertation Award from Penn Engineering, IBM Faculty Award, as well as six Best Paper and Runner-up Awards, such as the Best Paper Awards at the 2017 ACM SIGBED International Conference on Embedded Software (EMSOFT) and 2014 ACM/IEEE International Conference on Cyber-Physical Systems (ICCPS), and the Best Student Paper award at the 2012 IEEE Real-Time and Embedded Technology and Applications Symposium (RTAS). He is an associate editor in the ACM Transactions on Computing for Healthcare (ACM HEALTH) and a co-chair of the 2019 ACM/IEEE International Conference on Cyber-Physical Systems~(ICCPS'19).

% \end{IEEEbiography}


==> backup/Automatica_submission/commands.tex <==
\newcommand{\nat}{\mathbb{N}}

% \newcommand{\diag}{\mathcal{I}}

\renewcommand{\subset}{\subseteq }
\renewcommand{\supset}{\supseteq}
\renewcommand{\epsilon}{\varepsilon}

\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\c}{\circ}

\newcommand{\dom}{\mathrm{Dom}}
\newcommand{\image}{\mathrm{Image}}

\newcommand{\re}{\mathrm{Re}}

\newcommand{\rr}{\mathcal{R}}
\newcommand{\id}{\mathcal{I}}

\newcommand{\attacker}{\mathcal{A}}
\newcommand{\plant}{\mathcal{P}}
\newcommand{\supervisor}{\mathcal{S}}
\newcommand{\desired}{\mathscr{K}}

\newcommand{\astate}{\mathsf{s}}
\newcommand{\astates}{\mathsf{S}}
\newcommand{\ainit}{\mathsf{s}_\mathrm{init}}
\newcommand{\atransitions}{\mathsf{Trans}}
\newcommand{\aobservations}{\mathsf{Obs}}
\newcommand{\ainput}{\mathsf{i}}
\newcommand{\ainputs}{\mathbf{I}}
\newcommand{\aoutput}{\mathsf{o}}
\newcommand{\aoutputs}{\mathbf{O}}
\newcommand{\alabeling}{\mathsf{L}}
\newcommand{\afinal}{\mathsf{S}_\mathrm{final}}

\newcommand{\reach}{\mathsf{Reach}}

\newcommand{\ltrue}{\mathrm{True}}
\newcommand{\lfalse}{\mathrm{False}}
\newcommand{\lnext}{\mathbf{X}}
\newcommand{\luntil}{\mathbf{U}}
\newcommand{\lrelease}{\mathbf{R}}
\newcommand{\lfinal}{\mathbf{F}}
\newcommand{\lglobal}{\mathbf{G}}
\newcommand{\lall}{\mathbf{A}}
\newcommand{\lexist}{\mathbf{E}}
\newcommand{\lp}{\mathbf{P}}

\newcommand{\shift}{\mathcal{S}}
\newcommand{\iseq}[1]{#1^{(\infty)}}
\newcommand{\seq}[2]{#1^{(#2)}}
\newcommand{\set}[2]{\big\{ #1 \mid #2 \big\}}
\newcommand{\abs}[1]{\vert #1 \vert}
\newcommand{\argmax}{\mathrm{argmax}}


==> backup/Automatica_submission/desired_language.tex <==
\begin{tikzpicture}[>=latex,line join=bevel,scale=0.42]
%%
\begin{scope}
  \node (1) at (175.0bp,117.0bp) [draw,circle,double,solid] {$1$};
  \node (0) at (22.0bp,86.0bp) [draw,circle,double,initial,initial text=] {$0$};
  \node (3) at (175.0bp,55.0bp) [draw,circle,double,solid] {$3$};
  \node (2) at (328.0bp,146.0bp) [draw,circle,double,solid] {$2$};
  \node (5) at (481.0bp,118.0bp) [draw,circle,double,solid] {$5$};
  \node (4) at (328.0bp,84.0bp) [draw,circle,double,solid] {$4$};
  \node (7) at (481.0bp,56.0bp) [draw,circle,double,solid] {$7$};
  \node (6) at (328.0bp,22.0bp) [draw,circle,double,solid] {$6$};
  \node (8) at (634.0bp,87.0bp) [draw,circle,double,solid] {$8$};
\end{scope}
\begin{scope}
  \draw [->] (0) ..controls (48.209bp,77.754bp) and (53.78bp,76.221bp)  .. (59.0bp,75.0bp) .. controls (87.127bp,68.419bp) and (119.56bp,63.008bp)  .. (3);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (98.5bp,82.5bp) node {$t_{21}|t_{21}$};
  \draw [->] (3) ..controls (200.07bp,42.18bp) and (206.16bp,39.703bp)  .. (212.0bp,38.0bp) .. controls (239.59bp,29.952bp) and (272.07bp,25.913bp)  .. (6);
  \draw (251.5bp,45.5bp) node {$t_{22}|t_{22}$};
  \draw [->] (4) ..controls (373.45bp,91.063bp) and (411.63bp,97.717bp)  .. (444.0bp,106.0bp) .. controls (446.04bp,106.52bp) and (448.14bp,107.1bp)  .. (5);
  \draw (404.5bp,113.5bp) node {$t_{12}|t_{12}$};
  \draw [->] (5) ..controls (528.53bp,108.37bp) and (572.27bp,99.508bp)  .. (8);
  \draw (557.5bp,116.5bp) node {$t_{22}|t_{22}$};
  \draw [->] (4) ..controls (353.43bp,72.538bp) and (359.36bp,70.431bp)  .. (365.0bp,69.0bp) .. controls (392.77bp,61.958bp) and (425.24bp,58.729bp)  .. (7);
  \draw (404.5bp,76.5bp) node {$t_{22}|t_{22}$};
  \draw [->] (6) ..controls (373.94bp,24.515bp) and (412.29bp,28.368bp)  .. (444.0bp,38.0bp) .. controls (446.76bp,38.837bp) and (449.56bp,39.857bp)  .. (7);
  \draw (404.5bp,45.5bp) node {$t_{11}|t_{11}$};
  \draw [->] (7) ..controls (526.41bp,62.378bp) and (564.57bp,68.411bp)  .. (597.0bp,76.0bp) .. controls (599.04bp,76.477bp) and (601.13bp,77.002bp)  .. (8);
  \draw (557.5bp,83.5bp) node {$t_{12}|t_{12}$};
  \draw [->] (1) ..controls (201.18bp,107.98bp) and (206.76bp,106.32bp)  .. (212.0bp,105.0bp) .. controls (240.06bp,97.945bp) and (272.49bp,92.278bp)  .. (4);
  \draw (251.5bp,112.5bp) node {$t_{21}|t_{21}$};
  \draw [->] (3) ..controls (220.71bp,57.319bp) and (258.98bp,60.735bp)  .. (291.0bp,69.0bp) .. controls (293.47bp,69.637bp) and (295.99bp,70.4bp)  .. (4);
  \draw (251.5bp,76.5bp) node {$t_{11}|t_{11}$};
  \draw [->] (0) ..controls (69.534bp,95.631bp) and (113.27bp,104.49bp)  .. (1);
  \draw (98.5bp,115.5bp) node {$t_{11}|t_{11}$};
  \draw [->] (2) ..controls (375.94bp,137.23bp) and (419.53bp,129.25bp)  .. (5);
  \draw (404.5bp,145.5bp) node {$t_{21}|t_{21}$};
  \draw [->] (1) ..controls (222.94bp,126.09bp) and (266.53bp,134.35bp)  .. (2);
  \draw (251.5bp,145.5bp) node {$t_{12}|t_{12}$};
\end{scope}
%
\end{tikzpicture}

==> backup/Automatica_submission/input_attack.tex <==
\subsection{Supervisor Design Resilient to Actuator Attacks}
\label{sub:actuator attacks}

Unlike sensor attacks, {designing FST-based supervisors that are resilient to actuator attacks is not always possible (even if they can revise undesirable symbols).
% when FSTs are used to capture the supervisor's functionality.
}
% \todo{check} 
For example, if no actuation symbols are updated (i.e., the attacker $\attacker_a$ blocks all symbols from the supervisor $\plant$ in the control loop of Fig.~\ref{fig:control}), designing a resilient supervisor is impossible for any desired language $\desired$ (except for $\desired = \{\epsilon\}$). In this example, the infeasibility of resilient supervisors is caused by the restriction of the output language $L_{\mathrm{out}} (\attacker_a)$; to rule out this trivial case, we make the following technical assumption (otherwise, we can consider $\desired \cap L_{\mathrm{out}} (\attacker_a)$ instead of $\desired$).

\begin{assumption}
The output language of the attacks $\attacker_a$, in Fig.~\ref{fig:control}, contains the desired language $\desired$, i.e., $\desired \subseteq L_{\mathrm{out}} (\attacker_a)$.
\end{assumption}

Even under the above assumption, designing a resilient supervisor may still be unfeasible. 
Below, we present the condition for the design of attack-resilient supervisors for actuator attacks.


\begin{theorem}
\label{prop:actuator attack}
Without sensor attacks (in Fig.~\ref{fig:control}), for any plant $\plant$ and desired (prefix-closed regular) language $\desired \subseteq L_{\mathrm{in}}(\plant)$, the FST 
$$\supervisor = \plant^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1}$$
is a weakly-resilient supervisor (to the actuator attack $\attacker_a$) with
$$L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a) = \rr_{\attacker_a^{-1} \c \attacker_a} (\desired).$$
Particularly, $\supervisor$ is a resilient supervisor iff 
% \todo{just if? not iff?}
$$\rr_{\attacker_a^{-1} \c \attacker_a} (\desired) = \desired.$$
\end{theorem}


\begin{proof}
We defer the proof until Theorem 3.
% It suffices to show the language sent to the plant is exactly $\rr_{\attacker_a^{-1} \c \attacker_a} (\desired)$ under the supervisor $\supervisor = \plant^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1}$. Since 
% $$L_{\mathrm{out}} (\supervisor \c \attacker_a) \subseteq L_{\mathrm{out}} (\mathcal{M}_\desired \c {\attacker_a^{-1}} \c {\attacker_a}) \subseteq \rr_{\attacker_a^{-1} \c \attacker_a} (\desired),$$ 
% the plant only receives words in $\rr_{\attacker_a^{-1} \c \attacker_a} (\desired)$. On the other hand, for any $I \in \rr_{\attacker_a^{-1} \c \attacker_a} (\desired)$, from Lemma~\ref{lem:id} it holds that
% \yw{\[
% \begin{split}
% & I \in \rr_{\attacker_a^{-1} \c \attacker_a} (I) \subseteq \rr_{\plant \c \plant^{-1}} \c \rr_{\mathcal{M}_\desired} \c \rr_{\attacker_a^{-1} \c \attacker_a} (I)
% \\ & \quad = \rr_{\plant \c \plant^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1} \c \attacker_a} (I) = \rr_{\plant \c \supervisor \c \attacker_a} (I).
% \end{split}
% \]}
% Thus, the word $I$ can be sent to the plant.


% We now show the minimality of $L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a)$. Suppose there is another weakly-resilient supervisor $\supervisor'$ such that
% \begin{equation} \label{eq:pf_1}
%   \desired \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor', \attacker_a)  \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a).
% \end{equation}
% For simplicity, let $L' = L_{\mathrm{in}}(\plant \ \vert \ \supervisor', \attacker_a)$.
% For any input word $I' \in L'$ of the plant, there exists an output word $I$ of the supervisor such that $I \in \rr_{\attacker_a^{-1}} (I')$.
% For the word $I$, any revision by the attacker $\attacker_a$ can possibly be sent to the plant, so we have $\rr_{\attacker_a} (I) \subseteq L'$. Therefore, we have
% \begin{equation} \label{eq:pf_2}
%   \rr_{\attacker_a^{-1} \c {\attacker_a}} (L') \subseteq L'
% \end{equation}
% Combining \eqref{eq:pf_1} and \eqref{eq:pf_2}, we have $L' = \rr_{\attacker_a^{-1} \c \attacker_a} (\desired)$ since
% $\rr_{\attacker_a^{-1} \c {\attacker_a}} (\desired) \subseteq \rr_{\attacker_a^{-1} \c {\attacker_a}} (L') \subseteq L'$. 
\end{proof}



Intuitively, in the supervisor $\supervisor = \plant^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1}$, the part $\plant^{-1}$ partially recovers the plant's input from the output, then the part $\mathcal{M}_\desired$ filters out undesirable words, and finally the part $\attacker_a^{-1}$ prepares (not perfectly) for the attacks of $\attacker_a$. Theorem~\ref{prop:actuator attack} also directly leads to a  method for design of  supervisors resilient to actuator attacks, summarized in Algorithm~\ref{alg:actuator attack}.







\begin{algorithm}[!t]
\yw{
\caption{Resilient supervisor for actuator attacks}
\label{alg:actuator attack}
\begin{algorithmic}[1]
\Require{Plant $\plant$, desired language $\desired \subseteq L_{\mathrm{in}}(\plant)$, and actuator attacker $\attacker_a$.}

\State{Build an automaton $\mathcal{M}_\desired$ for $\desired$.}

\State{Compute inversions $\attacker_a^{-1}$, $\plant^{-1}$.}

\State{Compute serial composition $\supervisor =  \plant^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1}$.}


\If{$\rr_{\attacker_a^{-1} \c \attacker_a} (\desired) = \desired$}

\State \Return $\supervisor$ is a resilient supervisor.

\Else

\State \Return $\supervisor$ is a weakly-resilient supervisor.

\EndIf

\end{algorithmic}
}
\end{algorithm}







\begin{example}
\label{ex:input_attack}
Without sensor attacks (in Fig.~\ref{fig:control}), consider:
% \begin{itemize}
%   \item 
  a set of symbols $\ainputs = \{\ainput_1,\ainput_2\}$;
%   \item 
  a plant $\plant$ with input language $[\ainput_1, \ainput_2]^*$ as shown in Fig.~\ref{fig:input_plant}; and
%   \item 
  a desired language $\desired = \overline{[\ainput_1, \ainput_2] \ainput_2}$ modeled by automaton $\mathcal{M}_\desired$ in Fig.~\ref{fig:input_desired}.
% \end{itemize}
%
For the actuator attacks $\attacker_a$ from Fig.~\ref{fig:input_attack_1} that rewrite the first $\ainput_1$ nondeterministically to $\ainput_1$ or $\ainput_2$, the supervisor in Fig.~\ref{fig:input_supervisor_1} derived by Algorithm~\ref{alg:actuator attack} is resilient. 

For the actuator attacks $\attacker_a$ from Fig.~\ref{fig:input_attack_2} that rewrite any $\ainput_1$ nondeterministically to $\ainput_1$ or $\ainput_2$, the supervisor shown in Fig.~\ref{fig:input_supervisor_1} derived by Algorithm~\ref{alg:actuator attack} is weakly resilient and the minimal super-language is $\overline{[\ainput_1, \ainput_2] [\ainput_1, \ainput_2]}$. The supervisor cannot achieve exactly the desired language $\overline{[\ainput_1, \ainput_2] \ainput_2}$ which requires the second symbol to be $\ainput_2$ because the attacker $\attacker_a$ can always rewrite it to $\ainput_1$. 
\end{example}

\begin{figure}
\centering
\subcaptionbox{Plant.\label{fig:input_plant}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (s) {$0$};
  \path[->] (s) edge[loop right] node {\begin{minipage}{12pt}$\ainput_1 \vert \ainput_1$\\$\ainput_2 \vert \ainput_2$\end{minipage}} ();
\end{tikzpicture}
}
\subcaptionbox{Automaton of $\desired$.\label{fig:input_desired}}[.5\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0] (1) {$1$};
  \node[state,right of=1] (2) {$2$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1$} (1)
  (0) edge[bend right] node[below] {$\ainput_2$} (1)
  (1) edge[bend left] node[above] {$\ainput_2$} (2);

  % \path[->] (0) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1$} (1)
  % (0) edge[bend right] node[below] {$\ainput_2 \vert \ainput_2$} (1)
  % (1) edge[bend left] node[above] {$\ainput_1 \vert \epsilon$} (2)
  % (1) edge[bend right] node[below] {$\ainput_2 \vert \ainput_2$} (2)
  % (2) edge[loop right] node[right] {$\ainput_1, \ainput_2 \vert \epsilon$} (2);
\end{tikzpicture}
}


\par\bigskip
\subcaptionbox{Actuator Attacker I.\label{fig:input_attack_1}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0] (1) {$1$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1$} (1)
  (0) edge[bend right] node[below] {$\ainput_1 \vert \ainput_2$} (1)
  (1) edge[loop right] node[right] {\begin{minipage}{0pt}$\ainput_1 \vert \ainput_1$\\$\ainput_2 \vert \ainput_2$\end{minipage}} (1);
\end{tikzpicture}
}
\hspace{0.2cm}
\subcaptionbox{Supervisor I.\label{fig:input_supervisor_1}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0] (1) {$1$};
  \node[state,right of=1] (2) {$2$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1$} (1)
  (0) edge[bend right] node[below] {$\ainput_2 \vert \ainput_1$} (1)
  (1) edge[bend left] node[above] {$\ainput_2 \vert \ainput_2$} (2);
\end{tikzpicture}
}


\par\bigskip
\subcaptionbox{Actuator Attacker II.\label{fig:input_attack_2}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \path[->] (0) edge[loop above] node {$\ainput_1, \ainput_2 \vert \ainput_1, \ainput_2$} (0);
\end{tikzpicture}
}
\subcaptionbox{Supervisor II.\label{fig:input_supervisor_2}}[.5\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0,xshift=0.3cm] (1) {$1$};
  \node[state,right of=1,xshift=0.3cm] (2) {$2$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1, \ainput_2$} (1)
  (0) edge[bend right] node[below] {$\ainput_2 \vert \ainput_1, \ainput_2$} (1)
  (1) edge[bend left] node[above] {$\ainput_2 \vert \ainput_1, \ainput_2$} (2);
  % (1) edge[bend right] node[below] {$\ainput_2 \vert \ainput_1, \ainput_2$} (2);
\end{tikzpicture}
}
\caption{Example supervisors for actuator attacks.\label{fig:input_example}}
\end{figure}





==> backup/Automatica_submission/input_attacker.tex <==
\begin{tikzpicture}[>=latex,line join=bevel,scale=0.55]
%%
\node (1) at (188.5bp,91.499bp) [draw,ellipse,solid] {$1$};
  \node (0) at (39.5bp,59.499bp) [draw,circle, double,initial,initial text=] {$0$};
  \node (2) at (188.5bp,26.499bp) [draw,ellipse,solid] {$2$};
  \draw [->] (1) ..controls (167.45bp,79.965bp) and (161.35bp,77.272bp)  .. (155.5bp,75.499bp) .. controls (128.0bp,67.165bp) and (95.502bp,63.156bp)  .. (0);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (116.0bp,82.999bp) node {$t_{21}|t_{11}$};
  \draw [->] (0) ..controls (59.361bp,83.934bp) and (67.463bp,90.902bp)  .. (76.5bp,94.499bp) .. controls (103.77bp,105.35bp) and (137.8bp,102.37bp)  .. (1);
  \draw (116.0bp,109.0bp) node {$t_{11}|t_{21}$};
  \draw [->] (0) ..controls (64.579bp,46.698bp) and (70.668bp,44.216bp)  .. (76.5bp,42.499bp) .. controls (104.32bp,34.311bp) and (137.29bp,30.246bp)  .. (2);
  \draw (116.0bp,49.999bp) node {$t_{12}|t_{22}$};
  \draw [->] (2) ..controls (167.91bp,13.827bp) and (161.64bp,10.987bp)  .. (155.5bp,9.499bp) .. controls (121.38bp,1.2264bp) and (107.85bp,-6.304bp)  .. (76.5bp,9.499bp) .. controls (67.267bp,14.152bp) and (59.765bp,22.319bp)  .. (0);
  \draw (116.0bp,16.999bp) node {$t_{22}|t_{12}$};
  \draw [->] (0) ..controls (35.659bp,91.062bp) and (36.828bp,99.499bp)  .. (39.5bp,99.499bp) .. controls (41.17bp,99.499bp) and (42.253bp,96.203bp)  .. (0);
  \draw (-3.5bp,91.0bp) node {$t_{11}|t_{11}$};
  \draw [->] (0) ..controls (30.882bp,98.805bp) and (32.895bp,117.5bp)  .. (39.5bp,117.5bp) .. controls (44.867bp,117.5bp) and (47.202bp,105.16bp)  .. (0);
  \draw (-3.5bp,109.0bp) node {$t_{12}|t_{12}$};
  \draw [->] (0) ..controls (26.033bp,105.8bp) and (28.59bp,135.5bp)  .. (39.5bp,135.5bp) .. controls (49.004bp,135.5bp) and (52.169bp,112.96bp)  .. (0);
  \draw (-3.5bp,127.0bp) node {$t_{21}|t_{21}$};
  \draw [->] (0) ..controls (21.168bp,112.13bp) and (24.062bp,153.5bp)  .. (39.5bp,153.5bp) .. controls (53.37bp,153.5bp) and (57.115bp,120.11bp)  .. (0);
  \draw (-5.5bp,145.0bp) node {$t_{22}|t_{22}$};
%
\end{tikzpicture}

==> backup/Automatica_submission/intro.tex <==
\section{Introduction}
\label{sec:intro}


Supervisory control is a widely-used control architecture for cyber-physical systems (CPS) in various application domains including transportation~\cite{shepard12,pajic_csm17}, smart infrastructure~\cite{cassandras_SmartCitiesCyberPhysical_2016}, manufacturing~\cite{stuxnet,stuxnet2}, and healthcare~\cite{jiang_pieee12}. Specifically, the physical plant is abstracted by a finite-state model whose transitions are driven/observed through a set of discrete actuating/sensing symbols, whereas the supervisory controls the plant execution by monitoring and manipulating the discrete symbols.
% \todo{fix the "preliminary results appeared in " -- add both CDC papers}


As CPS are increasingly being used in potentially contested scenarios, such as autonomous driving~\cite{raman_ReactiveSynthesisSignal_2015,pajic_csm17} and distributed manufacturing~\cite{jakovljevic2019distributing,lesi2020security},  there is a growing interest in ensuring the resilience of supervisors against sensor/actuator attacks~\cite{lin2019towards,lima2019security,meira2021synthesis}. In this work, we consider a general closed-loop setup of supervisory control in the presence of attacks, illustrated in Fig.~\ref{fig:diagram}, where the sensing and actuating symbols from/to the plant may be corrupted by an attacker. To achieve attack-resilience, the supervisor aims to restrict the input \emph{words} (i.e., the sequence of actuating symbols) of the plant to some desired \emph{language} (i.e., a given set of desired words) even in the presence of (simultaneous) attacks on the sensors and actuators. Our setup captures most forms of malicious activity in CPS, possibly resulting from network-based attacks that corrupt the data communicated between the plant and supervisor (e.g.,~as in~\cite{smith_decoupled_attack,ncs_attack_models,jovanov_tac19,lesi_tecs17}), as well as non-invasive sensing attacks  (e.g.,~GPS spoofing attacks on autonomous vehicles~\cite{spoofedgps,warner2002simple} or Anti-lock Braking Systems (ABS) in cars~\cite{shoukry2013non}). This is more general than~\cite{wakaiki_SupervisoryControlDiscreteevent_2017} studying only sensor attacks and \cite{carvalho_DetectionMitigationClasses_2018} studying either sensor or actuator~attacks.


We define and study a general class of \emph{regular-rewriting} attacks, where the attackers can nondeterministically rewrite (e.g., insert, delete, and replace) sensing and actuating symbols using a given \emph{regular relation}. The regular relations are motivated by the constraints from common security measures in CPS. For example,~built-in intrusion detection systems (IDS)~\cite{bozkurt2020secure} memorize past symbols and raise an alarm if some symbols appear too often; to avoid easy detection, the attacker needs to constrain the pattern of its attack behavior based on history. Besides, intermittently authentication services constrain how frequent the attacks may happen~\cite{jovanov_tac19,lesi_rtss17,wang2019attack}. These history-dependent constraints can be mathematically captured by regular relations. The regular-rewriting attacks generalize previously studied nondeterministic and history-independent attacks~\cite{wakaiki_SupervisoryControlDiscreteevent_2017,su_SupervisorSynthesisThwart_2018,goes_StealthyDeceptionAttacks_2017,carvalho_DetectionMitigationClasses_2018}. Furthermore, the ability to capture history-dependence also allows for capturing of finite-memory replay attacks~\cite{stuxnet,stuxnet2}, which has not been studied in the domain of supervisory control of discrete-event systems. 
% \todo{added check} 


\yw{Previously, most works deal with supervisory control under attacks by directly analyzing the attackers' behavior~\cite{lin2019towards,lima2019security,meira2021synthesis}. In this work, we provide a model-based approach to elegantly capture the attackers' behavior and synthesis resilient supervisors.}
Specifically, we use nondeterministic-in-input finite-state transducers (FSTs)~\cite{sakarovitch_ElementsAutomataTheory_2003,droste_HandbookWeightedAutomata_2009} to model regular-rewriting attacks constrained by regular relations. FSTs can be viewed as automata that have both input and output symbols on their transitions. They are commonly used to model control programs or language models that generate different outputs based on past inputs~\cite{mohri_FiniteStateTransducersLanguage_1997,mohri_WeightedFinitestateTransducers_2002,mohri_WeightedFiniteStateTransducer_2004,mohri_WeightedAutomataAlgorithms_2009}. Here, the nondeterminism-in-input of the FSTs enables capturing of all the possible (maybe infinitely-many) attack behaviors under the regular relations. The advantages of using FST are twofold. First, FSTs are closed under inversion and composition, and thus multiple sources of attacks can be combined and modeled by a single FST. Second, common operations of FSTs (e.g., inversion, composition) are well-defined and supported by existing C\texttt{++}/Python libraries (e.g.,~\cite{openfst}).
% \todo{add citation}


We model the plant by nondeterministic-in-input FSTs as well, to also capture plants that can generate sensing symbols that are different from the actuation symbols. The nondeterminism allows us to capture the plant's internal faults or disturbance (not caused by attacks). This {generalizes previous works on attack-resilient supervisory control in which only deterministic plants are considered}~\cite{wakaiki_SupervisoryControlDiscreteevent_2017,su_SupervisorSynthesisThwart_2018,goes_StealthyDeceptionAttacks_2017,carvalho_DetectionMitigationClasses_2018}. Our plant modeling is similar to~\cite{xu2009discrete,ushio2015nonblocking}, although no attacks were considered in those~works.
% \todo{can we add something that if the considered setup is more general and also covers commonly considered deterministic plants?}


We consider a general class of supervisors that can rewrite symbols based on past observations considering that the rewriting ability is essential to defend against the regular-rewriting attacks. Mathematically, such supervisors can be modeled by FSTs. The supervisor's goal is to maintain the plant's execution (specifically, the plant's input word) to some desired language even under given regular-rewriting attacks on sensors and actuators. Similar to the classical supervisory control~\cite{cassandras_IntroductionDiscreteEvent_2008}, the FST-based supervisor can capture all control words that can incur desirable executions of the plant under attacks. The considered supervisor model is more powerful than the ones used in classical supervisory control~\cite{cassandras_IntroductionDiscreteEvent_2008} that can only allow/disallow symbols. It is more similar to the ones used for reactive synthesis and runtime enforcement~\cite{bloem2015shield}. 
% When the FST-based supervisor does not insert/replace symbols, our formulation reduces to classical supervisory control, as discussed in Section~\ref{rem:recover}.


We present new resilience conditions as well as algorithms to design resilient supervisors (for a given desired language of the plant) for given FST-based sensor and actuator attacks. Specifically, we show that the supervisor can be designed separately for actuator and sensor attacks. For both sensor and actuator attacks, the best countermeasure is to use the inversion of their FST models. The supervisor design is feasible if and only if the desired language is invariant under the composing of the actuator attack and its inversion. Furthermore, we present a tool for designing such attack-resilient supervisors and demonstrate its applicability on several case studies.


The paper is organized as follows. We provide preliminaries on FSTs and regular relations in Section~\ref{sec:prelim} and formalize the problem in Section~\ref{sec:formulation}. Then, we demonstrate the advantages of using FSTs to model attacks in Section~\ref{sec:attack} and provide resiliency conditions and algorithms to design resilient supervisors for FST-based sensor and actuator attacks in Section~\ref{sec:attack}. Finally, case studies are presented in Section~\ref{sec:sim}, before concluding in Section~\ref{sec:conclusion}.


\begin{figure}[!t]
\usetikzlibrary{arrows}
\centering
\begin{tikzpicture}
\draw[black] (0,0) rectangle (6,.5);
\draw [dotted] (1.5, 0) -- (1.5, 0.5);
\draw [dotted] (4.5, 0) -- (4.5, 0.5);
\draw[black] (1.5,2) rectangle (4.5,2.5);
\draw [dotted, rounded corners] (0, 1) rectangle (6,1.5);

\draw [->, >=latex] (0.75, 0.5) -- (0.75,1.35);
\draw (0.75,1.3) -- (0.75,2.25);
\draw (0.75,2.25) -- (1.5,2.25);
\draw (4.5,2.3) -- (5.25,2.3);
\draw [->, >=latex] (5.25,2.3) -- (5.25,1.2);
\draw (5.25,1.25) -- (5.25,0.5);

\draw [->,dashed, >=stealth] (6,2.5) -- (5.35, 1.5);
\draw [->,dashed, >=stealth] (6,2.5) -- (5.35, 0.5);

\draw [->,dashed, >=stealth] (0,2.5) -- (0.65, 1.5);
\draw [->,dashed,  >=stealth] (0,2.5) -- (0.65, 0.5);

\node at (3,0.25) {Plant};
\node at (5.25,0.25) {Actuator};
\node at (0.75,0.25) {Sensor};
\node at (3,1.25) { Communication Network};
\node at (3,2.25) {Supervisor};

\node[align=center] at (6,3) {\small Actuator \\ \small Attacks};
\node[align=center] at (0,3) {\small Sensor \\ \small Attacks};
\end{tikzpicture}
\caption{Considered control architecture capturing attacks on sensing and actuation data between the plant and supervisor.} \label{fig:diagram}
\end{figure}









==> backup/Automatica_submission/io_attack.tex <==
\section{Attack-Resilient Supervisor Design}
\label{sec:design}

Following the problem formulation in Section~\ref{sec:formulation}, in this section we focus on the design of supervisors under sensor and actuator attacks. We proceed by studying attacks 1) only on sensors, 2) only on actuators, and 3) on both sensors and actuators.


\input{output_attack}
\input{input_attack}


\subsection{Design of Supervisors Resilient to Sensor and Actuator Attacks}

When both sensor and actuator attacks may occur in the system, we combine Theorems~\ref{prop:sensor attack} and~\ref{prop:actuator attack}. From Theorem~\ref{prop:sensor attack}, sensor attacks have little influence on the feasibility of designing resilient attacks. Thus, the conditions for designing resilient supervisors under both attacks are similar to the conditions from Theorem~\ref{prop:sensor attack} that only consider actuator attacks.
% \todo{check}
% \todo{why is this a theorem and other propositions? it's weird to have 1 theorem in an Automatica paper + it's not much more complex. make all these theorems + check for consistency over the paper as you used hard-coded words for Theorem/Proposition}


\yw{
\begin{theorem}
\label{thm:both attack}
For systems from Fig.~\ref{fig:control}, for any plant $\plant$ and desired (prefix-closed regular) language $\desired \subseteq L_{\mathrm{in}}(\plant)$, the FST 
$$\supervisor=\attacker_s^{-1} \c \plant^{-1} \c \mathcal{M}_\desired \c {\attacker_a^{-1}}$$
is a weakly-resilient supervisor (to the attacks $\attacker_a$ and $\attacker_s$) with
$$L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a, \attacker_s) = \rr_{\attacker_a^{-1} \c \attacker_a} (\desired).$$
Particularly, $\supervisor$ is a resilient supervisor iff 
% \todo{comment on why not necessary and sufficient}
$$\rr_{\attacker_a^{-1} \c \attacker_a} (\desired) = \desired.$$
\end{theorem}


\begin{proof} It suffices to show the language sent to the plant is exactly $\rr_{\attacker_a^{-1} \c \attacker_a} (\desired)$ under the supervisor $\supervisor=\attacker_s^{-1} \c \plant^{-1} \c \mathcal{M}_\desired \c {\attacker_a^{-1}}$. Since $L_{\mathrm{out}} (\supervisor \c {\attacker_a}) \subseteq  L_{\mathrm{out}} (\mathcal{M}_\desired \c {\attacker_a^{-1}} \c {\attacker_a}) \subseteq \rr_{\attacker_a^{-1} \c \attacker_a} (\desired)$, the plant only receives words in $\rr_{\attacker_a^{-1} \c \attacker_a} (\desired)$.
%
On the other hand, for any $I \in \desired$, we have by Lemma~\ref{lem:id}
\[
\begin{split}
& I \in \rr_{\attacker_a^{-1} \c \attacker_a} (I) \subseteq \rr_{(\plant \c \attacker_s) \c (\plant \c \attacker_s)^{-1}} \c \rr_{\mathcal{M}_\desired} \c \rr_{\attacker_a^{-1} \c \attacker_a} (I)
\\ & \quad = \rr_{\plant \c \attacker_s \c (\plant \c \attacker_s)^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1} \c \attacker_a} (I) = \rr_{\plant \c \attacker_s \c \supervisor \c \attacker_a} (I).
\end{split}
\]}
So the word $I$ can be sent to the plant.

The minimality of $L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a, \attacker_s)$ can be proved in the same way as Theorem~\ref{prop:actuator attack}.
\end{proof}


Theorem~\ref{thm:both attack} also directly provides a design method for resilient supervisors to the actuator and sensor attacks, as captured in Algorithm~\ref{alg:both attack}. We provide an example below.


\begin{algorithm}[!t]
\caption{Resilient supervisor for actuator and sensor attacks}
\label{alg:both attack}
\yw{
\begin{algorithmic}[1]

\Require{Plant $\plant$, desired language $\desired \subseteq L_{\mathrm{out}}(\plant)$, and attackers $\attacker_s$ and $\attacker_a$.}

\State{Build an automaton $\mathcal{M}_\desired$ for $\desired$.}

\State{Compute inversion $\attacker_a^{-1}$, $\plant^{-1}$ and $\attacker_s^{-1}$.}

\State{Compute composition $\supervisor = \attacker_s^{-1} \c \plant^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1}$.}

\If{$\rr_{\attacker_a^{-1} \c \attacker_a} (\desired) = \desired$}

\State \Return $\supervisor$ is a resilient supervisor.

\Else

\State \Return $\supervisor$ is a weakly-resilient supervisor.

\EndIf

\end{algorithmic}
}
\end{algorithm}










\begin{example}
\label{ex:both_attack}
Following Example~\ref{ex:input_attack}, consider extra sensor attacks modeled as in Fig.~\ref{fig:both_attack_1} and~\ref{fig:both_attack_2}. The supervisor in Fig.~\ref{fig:both_supervisor_1} derived by Algorithm~\ref{alg:both attack} is resilient to sensor attacks in Fig.~\ref{fig:both_attack_1} and the actuator attacks in Fig.~\ref{fig:input_attack_1}. The supervisor in Fig.~\ref{fig:both_supervisor_2} derived by Algorithm~\ref{alg:both attack} is resilient to sensor attacks in Fig.~\ref{fig:both_attack_2} and the actuator attacks in Fig.~\ref{fig:input_attack_2}. Comparing to Example~\ref{ex:input_attack}, the sensor attacks do not affect the {feasibility of attack-resilient supervisor design}.
% \todo{this is the first time you talk about controllability; say what it is} 
This agrees with results from Theorem~\ref{prop:actuator attack} and Theorem~\ref{thm:both attack}.
\end{example}










\begin{figure*}[!t]
\centering
\subcaptionbox{Sensor Attacker I\label{fig:both_attack_1}}[.2\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \path[->] (0) edge[loop above] node {\begin{minipage}{12pt}$\ainput_1 \vert \ainput_2$\\$\ainput_2 \vert \epsilon$\end{minipage}} (0);
\end{tikzpicture}
}
\subcaptionbox{Supervisor I\label{fig:both_supervisor_1}}[.2\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0] (1) {$1$};
  \node[state,right of=1] (2) {$2$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_2 \vert \ainput_1$} (1)
  (0) edge[bend right] node[below] {$\epsilon \vert \ainput_1$} (1)
  (1) edge[bend left] node[above] {$\epsilon \vert \ainput_2$} (2);
\end{tikzpicture}
}
\subcaptionbox{Sensor Attacker II\label{fig:both_attack_2}}[.2\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \path[->] (0) edge[loop above] node {$\ainput_1, \ainput_2\vert \ainput_2$} (0);
\end{tikzpicture}
}
\subcaptionbox{Supervisor II\label{fig:both_supervisor_2}}[.2\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0,xshift=0.3cm] (1) {$1$};
  \node[state,right of=1,xshift=0.3cm] (2) {$2$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_2 \vert \ainput_1, \ainput_2$} (1);
  \path[->] (1) edge[bend left] node[above] {$\ainput_2 \vert \ainput_1, \ainput_2$} (2);
\end{tikzpicture}
}
\caption{Example supervisors for both sensor and actuator attacks.\label{fig:both_example}}
\end{figure*}







\subsection{Relationship to Previous Work} \label{rem:recover}

Due to its generality, the presented FST-based framework described in Section~\ref{sec:formulation} and~\ref{sec:attack} %in Figure~\ref{fig:control} 
also covers several previously-studied setups of supervisory control -- i.e., the results derived in this section directly apply to them. Since we use FST-based supervisors (instead of automaton-based supervisors in those works), the designed supervisors may differ. 


The classical supervisory control~\cite{cassandras_IntroductionDiscreteEvent_2008} with uncontrollable symbols $\ainputs_{uc}$ %and unobservable symbols $\ainputs_{uo}$ 
can be formulated in our framework {by adopting the following setups in Fig.~\ref{fig:control}}.
% \todo{Figure 3 does not show a framework. it is a control diagram}  
\begin{itemize}
  \item[-] Let $\plant$ be the plant (an automaton) of interest.
  \item[-] Let the actuator attacker be $\attacker_a^{(s)} = \mathrm{Inject}_{\ainputs_{uc}} \circ \plant$ be the serial composition of the injection attack from~\eqref{eq:injection} and the plant. This attacker injects uncontrollable symbols in $\ainputs_{uc}$ whenever they are acceptable by the plant.
  % \item[-] Let the sensor attacker be $\attacker_s^{(s)}=\mathrm{Project}_{\ainputs \backslash \ainputs_{uo}}$ from~\eqref{eq:projection}, which removes unobservable symbols in $\ainputs_{uo}$.
\end{itemize}


Following the above formulation, the supervisory control under sensor/actuator enablement and disablement attacks~\cite{carvalho_DetectionMitigationClasses_2018} can be formulated in our framework %of Figure~\ref{fig:control} by
by
% \begin{itemize}[leftmargin=12pt]
%   \item[-] 
  letting the sensor/actuator attacks be $\attacker_a^{(ed)} \circ \attacker_a^{(s)}$, where $\attacker_a^{(s)}$ is defined above and $\attacker_a^{(ed)}$ is the injection-removal attack on a set of vulnerable control symbols from Example~\ref{ex:ins-rem}.
% \end{itemize}


Finally, the supervisory control under replacement-removal sensor attacks~\cite{wakaiki_SupervisoryControlDiscreteevent_2017} can be formulated in our framework % of Figure~\ref{fig:control} 
by
% \todo{you had itemized lists with a single item; unless you missed something, I've removed the list formatting}
% \begin{itemize}[leftmargin=12pt]
%   \item[-] 
letting the sensor attacks be $\attacker_s^{(rr)} \circ \attacker_s^{(s)}$, where $\attacker_s^{(s)}$ is defined above and $\attacker_s^{(rr)}$ is the replacement-removal attack from Example~\ref{ex:rep-rem}.
% \end{itemize}

==> backup/Automatica_submission/modeling.tex <==
\section{Problem Formulation}
\label{sec:formulation}

We aim to design a supervisor $\supervisor$ to control a given plant $\plant$ in the presence of given attackers $\attacker_a$ and $\attacker_s$ as shown in Fig.~\ref{fig:control}. The plant may have internal faults or disturbance (not caused by the attacks) and different input/output symbols, so we model it by an implementable nondeterministic FST. The supervisory control goal is to restrict the input words to the plant to a given regular language $\desired \subseteq L_{\mathrm{in}}(\plant)$.


We introduce a general class of regular-rewriting attacks for $\attacker_a$ and $\attacker_s$, which can nondeterministically rewrite (e.g., insert, delete, and replace) sensing/actuating symbols according to the observation/control history by a given regular relation. Mathematically, the attackers $\attacker_a$ and $\attacker_s$ are modeled by two given implementable nondeterministic FSTs, where the nondeterminism captures all the possible (maybe infinitely-many) attack behaviors under the regular relations. 

We consider a class of supervisors that can rewrite actuating symbols based on past sensing symbols since this ability is essential to counter regular-rewriting attacks. Mathematically, the supervisor $\supervisor$ is modeled by an implementable FST. It is more powerful than classical ones~\cite{cassandras_IntroductionDiscreteEvent_2008} that can only allow/disable symbols and is more similar to the ones used in reactive synthesis and runtime enforcement~\cite{bloem2015shield}. 
Our formulation can reduce to the classical supervisory control setup~\cite{cassandras_IntroductionDiscreteEvent_2008}, including the previous works on attack-resilient supervisory control~\cite{wakaiki_SupervisoryControlDiscreteevent_2017,su_SupervisorSynthesisThwart_2018,goes_StealthyDeceptionAttacks_2017,carvalho_DetectionMitigationClasses_2018} by choosing the corresponding forms of the FSTs $\attacker_a$ and $\attacker_s$ (discussed in~Section~\ref{rem:recover}). 
% \todo{to mention here that we will look at non-FST supervisors too?}


\begin{figure}[!t]
\centering
\begin{tikzpicture}
 \node (center) {};
 \node [draw, right of=center, node distance=1.5cm]  (ai) {Attacker $\attacker_a$};
 \node [draw, below of=center, node distance=1cm]  (p) {Plant $\plant$};
 \node [draw, left of=center, node distance=1.5cm] (ao) {Attacker $\attacker_s$};
 \node [draw, above of=center, node distance=1cm] (s) {Supervisor $\mathcal{S}$};

 \draw [->] (ai) |- node [below,right] {$\ainput_{\plant}$} (p);
 \draw [->] (p) -| node [below,left] {$\aoutput_{\plant}$} (ao);
 \draw [->] (ao) |- node [above,left] {$\ainput_{\supervisor}$} (s);
 \draw [->] (s) -| node [above,right] {$\ainput_{\supervisor}$}  (ai);
\end{tikzpicture}
\caption{Supervisory control under sensor and actuator attacks.\label{fig:control}}
\end{figure}


\yw{
To describe the evolution of the closed-loop system in Fig.~\ref{fig:control}, let us introduce an imaginary discrete-time global clock for the FSTs $\supervisor$, $\attacker_s$, $\attacker_a$, and $\plant$. At each clock instance, all FSTs can make at most one transition; the closed-loop system can make an evolution iff $\ainput_{\plant} | \aoutput_{\plant}$, $\aoutput_{\plant} | \ainput_{\supervisor} $, $\ainput_{\supervisor} | \aoutput_{\supervisor}$, and $\aoutput_{\supervisor} | \ainput_{\plant}$ are accepted by $\supervisor$, $\attacker_s$, $\attacker_a$, and $P$, respectively. We make the convention that  $\varepsilon | \varepsilon$ is accepted by any FST; this includes two cases: (i) there is an FST transition labeled by $\varepsilon | \varepsilon$ corresponds to a transition of the FST, or (ii) the FST makes no transition.



Equivalently, we can model the evolution of the closed-loop system as if driven by the supervisor. As shown in Fig.~\ref{fig:control}, the FST transitions of the supervisor can be viewed as successive automata transitions (by adding intermediate phantom states). At the state $\astate$, the supervisor triggers the evolution of the close loop system by sending a symbol $\ainput$ and moving to the phantom state $\astate$. After passing through the FSTs $\attacker_a$, $\plant$, and $\attacker_s$, the symbol $\ainput$ will be nondeterministically revised to another symbol $\aoutput$ and received by the supervisor. Then the supervisor will move (from the intermediate phantom state $\astate$) to the next state if the transition $(\astate_1, \ainput, \aoutput, \astate_2)$ is permitted. Otherwise, the evaluation will stop, and we undo the transitions of $\attacker_a$, $\plant$, and $\attacker_s$ cased by the symbol $\ainput$.

\begin{figure}[!t]
\centering
\subcaptionbox{\label{fig:split_1}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state] (0) {$\astate_1$};
  \node[state, right of=0, xshift=0.5cm] (1) {$\astate_2$};
  \path[->] (0) edge node[above] {$\ainput | \aoutput$} (1);
\end{tikzpicture}
}
\subcaptionbox{\label{fig:split_2}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state] (0) {$\astate_1$};
  \node[state, dashed, right of=0, xshift=0.5cm] (00) {$\astate$};
  \node[state, right of=00, xshift=0.5cm] (1) {$\astate_2$};
  \path[->] (0) edge node[above] {$\varepsilon | \aoutput$} (00);
  \path[->] (00) edge node[above] {$\ainput | \varepsilon $} (1);
\end{tikzpicture}
}
\caption{Viewing a transition of supervisor as two successive transitions\label{fig:split}}
\end{figure}
}


The closed-loop input language of the plant in Fig.~\ref{fig:control} (i.e., the set of all possible input words to the plant in the closed-loop system under the nondeterminism of $\plant$, $\supervisor$, $\attacker_s$, and $\attacker_a$) is denoted by $L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a, \attacker_s)$. We denote it as $L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a)$ or $L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_s)$ if there are only actuator or only sensor attacks, respectively.

\yw{
\begin{example}
Following the above supervisor-driven description of the closed-loop system in Fig.~\ref{fig:control}, suppose the plant and supervisor are the FSTs shown in Fig.~\ref{fig:closeloop}, and there is no attacker. At time step 1, the supervisor starts from state 0 and sends $\ainput_1$. The plant receives $\ainput_1$, sends $\ainput_1$, and moves (i.e., transitions) to state 1. Upon receiving $\ainput_1$, the supervisor moves to state 1. Then, at time step 2, the supervisor starts from state 1 and sends $\ainput_2$; the plant receives Symbol $\ainput_2$ and sends $\ainput_1$. Upon receiving $\ainput_1$, the supervisor moves back to state 0. The above steps are repeatable, so the input language of the plant is $L_\textrm{in} (P | S)=\ainput_1^*$.
\end{example}

\begin{figure}
\centering
\subcaptionbox{Plant $\plant$}[.45\linewidth]{
\begin{tikzpicture}
  \node[state, initial, initial text=] (s) {$0$};
  \path[->] (s) edge[loop right] node {$\ainput_1,\ainput_2 \vert \ainput_2$} ();
\end{tikzpicture}
}
\subcaptionbox{Supervisor $\supervisor$}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0, xshift=0.5cm] (1) {$1$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1$} (1)
  (1) edge[bend left] node[above] {$\ainput_1 \vert \ainput_2$} (0);
\end{tikzpicture}
}
\caption{Example of closed-loop system evolution.\label{fig:closeloop}}
\end{figure}
}


\begin{definition}
\label{def:controllability}
Given the plant $\plant$ and attackers $\attacker_s$ and $\attacker_a$ modeled by implementable nondeterministic FSTs, the implementable FST $\supervisor$ is a resilient supervisor (w.r.t. to the attack model) for a given desired language $\desired$ iff the closed-loop input language of the plant satisfies
\[
  \desired = L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a, \attacker_s).
\]
\end{definition}

Since designing a resilient supervisor is not always possible, we consider a related problem to design a weakly-resilient supervisor that achieves the minimal super-language of the desired language $\desired$. 
\yw{Generally, we view $\desired$ as the set of required executions of the plant (similar to the classical supervisory control theory~\cite{cassandras_IntroductionDiscreteEvent_2008}) and try to design a minimal supervisor that can fulfill this requirement under the sensor and actuating attacks. In addition, weak resiliency serves as a necessary condition for resiliency. In Section 5, we will show that designing a weakly resilient supervisor is always possible, and designing a resilient supervisor is possible if and only if the weakly resilient supervisor is resilient.}


\begin{definition}
\label{def:weak supervisor}
The FST $\supervisor$ is a weakly-resilient supervisor for a desired language $\desired$ iff
\begin{itemize}
  \item $\desired \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a, \attacker_s)$, and
  \item for any $\supervisor'$ that satisfies 
  $\desired \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor', \attacker_a, \attacker_s)$, it holds that 
  $L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a, \attacker_s) \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor', \attacker_a, \attacker_s)$.
\end{itemize}
\end{definition}


To simplify our presentation, we make the following two assumptions.


\begin{assumption}
For the plant $\plant$ and the attack models $\attacker_a$ and $\attacker_s$,
% \todo{how limiting these are?}
\begin{itemize}[leftmargin=10pt]
  \item[-] all states are final, i.e., their input and output languages are prefix-closed; the desired language $\desired$ is also prefix-closed and regular;
  \item[-] they only receive acceptable inputs, i.e., the attacks $\attacker_a$ and $\attacker_s$ only try to undermine the control of the plant by sending words in $L_{\mathrm{in}}(\plant) \backslash \desired$ to it.
\end{itemize}
\end{assumption}

{The first assumption is commonly adopted in existing work on attack-resilient supervisory control~\cite{wakaiki_SupervisoryControlDiscreteevent_2017,su_SupervisorSynthesisThwart_2018,goes_StealthyDeceptionAttacks_2017,carvalho_DetectionMitigationClasses_2018}.
The second assumption can always be satisfied by introducing additional transitions to an error state when the FST received unacceptable inputs.}

{In what follows, we will discuss how to model sensor and actuator attacks by FSTs (Section~\ref{sec:attack}), before showing how to design resilient supervisors under these attacks (in Section~\ref{sec:design}).

% \todo{here, pls add "in the next section we do... before in Sec cc we provide how,,,,}



==> backup/Automatica_submission/nondeterminism.tex <==
\subsection*{Implementability of FSTs}
Our framework allows nondeterministic FST to model the supervisor. Due to the nondeterminism, an acceptable pair input/output word is not always executable if sent symbol-by-symbol to the FST. For example, the FST in 
Fig.~\ref{fig:non_imp} allows input $\ainput_1 \ainput_2$ and output $\ainput_2 \ainput_3$ through following the state transitions $0 \to 1 \to 3$. However, if the FST first receives the input symbol $\ainput_1$ and output symbol $\ainput_2$ and then jumps to the state $2$, then the rest of the input and output symbols are not executable any more.


For example, the FST in Fig.~\ref{fig:non_imp} is non-implementable; when executing the word $\ainput_1 \ainput_2$ symbol-by-symbol, if it transits from the state $0$ to the state $2$ upon receiving the first symbol $\ainput_1$, then next symbol $\ainput_2$ will be blocked. This is captured as follows.

\begin{figure}[!t]
\centering
\subcaptionbox{Non-implementable FST.\label{fig:non_imp}}[.5\linewidth]{
\begin{tikzpicture}
	\node[state,initial, initial text=] (0) {$0$};
	\node[state,right of=0, xshift=0.4cm, yshift=0.5cm] (1) {$1$};
	\node[state,right of=0, xshift=0.4cm, yshift=-0.5cm] (2) {$2$};
	\node[state,right of=0, xshift=2cm] (3) {$3$};
	\path[->] (0) edge node[above] {$\ainput_1 \vert \ainput_2$} (1);
	\path[->] (0) edge node[below] {$\ainput_1 \vert \ainput_2$} (2);
	\path[->] (1) edge node[above] {$\ainput_2 \vert \ainput_3$} (3);
	\path[->] (2) edge node[below] {$\ainput_3 \vert \ainput_3$} (3);
\end{tikzpicture}
}
\subcaptionbox{Determinization.\label{fig:determinization}}[.48\linewidth]{
\begin{tikzpicture}
\node[state, initial, initial text=] (0) {$0$};
\node[state, right of=0, xshift=0.2cm] (1) {$1,2$};
\node[state, right of=1, xshift=0.2cm] (2) {$3$};
\path[->] (0) edge node[above] {$\ainput_1 \vert \ainput_2$} (1);            
\path[->] (1) edge[bend left] node[above] {$\ainput_2 \vert \ainput_3$} (2);                 
\path[->] (1) edge[bend right] node[below] {$\ainput_3 \vert \ainput_3$} (2);
\end{tikzpicture}
}
\caption{Examples of checking FST implementability.}
\end{figure}




\begin{definition}
\label{def:implementable}
An FST $\attacker = (\astates, \ainit, \allowbreak \ainputs, \aoutputs, \atransitions, \afinal)$ is implementable iff
\begin{align*}
& \forall I \in L_{\mathrm{in}} (\attacker) \ \forall i \in \ainputs.
\Big( \exists \astate \in \reach_\attacker (I). \ \atransitions(\astate, \ainput, \cdot, \cdot)  
\\ & \neq \emptyset \Big) \implies
\Big( \forall \astate \in \reach_\attacker (I). \ \atransitions(\astate, \ainput, \cdot, \cdot) \neq \emptyset \Big)  
\end{align*}
where $\reach_\attacker (I)$ is the reachset of the {input} word 
% \todo{Check} 
$I$. 
\end{definition}

Definition~\ref{def:implementable} means that if an input symbol is enabled on a state of $\astate \in \reach_\attacker (I)$ then it should be also enabled on all states of $\astate \in \reach_\attacker (I)$. It ensures that every enabled symbol can be executed regardless of the FST's past (nondeterministic) executions. For deterministic FSTs, $\abs{\reach_\attacker (I)}=1$ for any $I \in L_{\mathrm{in}} (\attacker)$, and thus the following lemma directly holds.
% \todo{check}

\begin{lemma}
Deterministic FSTs are implementable.
\end{lemma}

Checking implementability directly by Definition~\ref{def:implementable} is impractical, as it requires evaluating the above condition for all $I \in L_{\mathrm{in}} (\attacker)$. To resolve this issue, we introduce the input-determinization for FSTs based on the powerset construction for automata~\cite{sipser_IntroductionTheoryComputation_1996}.

\begin{definition}
The input-determinization of the FST $\attacker = (\astates, \ainit, \ainputs, \aoutputs, \atransitions, \afinal = \astates)$ 
is an automata $\attacker^D = (\astates^D, \ainit^D, \ainputs^D, \atransitions^D, \afinal^D = \astates^D)$ constructed as:  
\begin{itemize}[leftmargin=10pt]
\item[-] Let $\astates^D = 2^\astates$, $\ainit^D = \{\ainit\}$, and $\ainputs^D = \ainputs$.
\item[-] Let $(\astates_1, \ainput, \astates_2) \in \atransitions^D$ iff
\begin{itemize}
\item $\astates_1 \subseteq \astates$ and $\ainput \in \ainputs$, 
\item $\astate \in \astates_2$ iff there exists a sequence $(\astate_0, \ainput_1, \aoutput_1, \astate_1) \allowbreak ... (\astate_{n-1}, \ainput_n, \aoutput_n, \astate_n)$ with
\yw{$s_0 \in S_1$,
$s_n = s$, and} 
$(\astate_{i-1}, \ainput_i, \aoutput_i, \astate_i) \in \atransitions$ for $i \in [n]$ such that
$\ainput_1 ... \ainput_n = \ainput$ (i.e., one of $\ainput_1, ..., \ainput_n$ is $\ainput$ and all
% \todo{check}  
others are $\varepsilon$).
\end{itemize}
\item[-] Remove unreachable states (from $\ainit^D$) in $\astates^D$.
\end{itemize}
\end{definition}


The states of $\attacker^D$ are the powerset of the states of $\attacker$. Both $\attacker$ and $\attacker^D$ take input symbols from $\ainputs$. A transition $(\astates_1, \ainput, \astates_2)$ exists in $\astates^D$ iff $\astates_2$ is exactly those states in $\attacker$ that can be reached from some state in $\astates_1$ by taking an input symbol $\ainput$ (maybe through multiple transition as there are transitions with $\varepsilon$ input). 


Following the same approach as in~\cite{sipser_IntroductionTheoryComputation_1996}, it holds that the automata $\attacker^D$ is deterministic and free from $\varepsilon$-moves. Besides, $\attacker^D$ defines the same regular relation as $\attacker$. 
Furthermore, 
\yw{due to the determinism of $\attacker^D$, for any input word $I$, the reachset $\reach_{\attacker^D} (I)$ is a singleton and equal to  
$\{\reach_\attacker(I)\}$.}
Since we have removed unreachable states in $\attacker^D$, when $I$ runs over $L_{\mathrm{in}} (\attacker)$, $\reach_\attacker(I)$ runs over all the states of $\attacker^D$. Thus, the following lemma holds.


\begin{lemma} \label{lem:check_implementable}
The {FST} $\attacker$
% \todo{why the plant?} 
is implementable iff
\begin{align*}
& \forall \astate^D \in \astates^D \ \forall i \in \ainputs.
\Big( \exists \astate \in \astate^D. \ \atransitions(\astate, \ainput, \cdot, \cdot)  
\\ & \neq \emptyset \Big) \implies
\Big( \forall \astate \in \astate^D. \ \atransitions(\astate, \ainput, \cdot, \cdot) \neq \emptyset \Big)  
\end{align*}
\end{lemma}

Lemma~\ref{lem:check_implementable} can be directly used to check implementability by enumerating over all $\astate^D \in \astates^D$, $i \in \ainputs$ and $\astate \in \astate^D$. %Below is an example.

\begin{example}
The automaton in Fig.~\ref{fig:determinization} is the input-determinization of the FST in Figure~\ref{fig:non_imp}. The two FST states $1$ and $2$ correspond to the same automaton state $1,2$, because they are both reachable for the input $\ainput_1$. The FST is not implementable because $i_2$ is enabled on its state $1$ but not state $2$.   
\end{example}


% \begin{assumption} \label{ass:implementable}
% In the rest of this paper, we focus on implementable FSTs.
% \todo{is this a limitation? if no, why? if yes, how we'll address it?}
% \end{assumption}

==> backup/Automatica_submission/output_attacker.tex <==
\begin{tikzpicture}[>=latex,line join=bevel,scale=0.6]
%%
\node (0) at (42.0bp,22.0bp) [draw,circle, double,initial,initial text=] {$0$};
  \draw [->] (0) ..controls (39.896bp,53.795bp) and (40.544bp,62.0bp)  .. (42.0bp,62.0bp) .. controls (42.887bp,62.0bp) and (43.475bp,58.953bp)  .. (0);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (12.0bp,59.5bp) node {$t_{11}|\epsilon$};
  \draw [->] (0) ..controls (37.263bp,61.724bp) and (38.391bp,80.0bp)  .. (42.0bp,80.0bp) .. controls (44.904bp,80.0bp) and (46.202bp,68.166bp)  .. (0);
  \draw (12.0bp,77.5bp) node {$t_{12}|\epsilon$};
  \draw [->] (0) ..controls (34.587bp,68.903bp) and (36.032bp,98.0bp)  .. (42.0bp,98.0bp) .. controls (47.175bp,98.0bp) and (48.949bp,76.119bp)  .. (0);
  \draw (12.0bp,95.5bp) node {$t_{21}|t_{21}$};
  \draw [->] (0) ..controls (31.917bp,75.815bp) and (33.592bp,116.0bp)  .. (42.0bp,116.0bp) .. controls (49.554bp,116.0bp) and (51.674bp,83.563bp)  .. (0);
  \draw (12.0bp,113.5bp) node {$t_{22}|t_{22}$};
%
\end{tikzpicture}

==> backup/Automatica_submission/plant.tex <==
\begin{tikzpicture}[>=latex,line join=bevel,scale=0.6]
%%
\node (0) at (39.5bp,22.0bp) [draw,circle, double,initial,initial text=] {$0$};
  \draw [->] (0) ..controls (37.396bp,53.795bp) and (38.044bp,62.0bp)  .. (39.5bp,62.0bp) .. controls (40.387bp,62.0bp) and (40.975bp,58.953bp)  .. (0);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (9.0bp,54.5bp) node {$t_{11}|t_{11}$};
  \draw [->] (0) ..controls (34.763bp,61.724bp) and (35.891bp,80.0bp)  .. (39.5bp,80.0bp) .. controls (42.404bp,80.0bp) and (43.702bp,68.166bp)  .. (0);
  \draw (9.0bp,72.5bp) node {$t_{12}|t_{12}$};
  \draw [->] (0) ..controls (32.087bp,68.903bp) and (33.532bp,98.0bp)  .. (39.5bp,98.0bp) .. controls (44.675bp,98.0bp) and (46.449bp,76.119bp)  .. (0);
  \draw (9.0bp,90.5bp) node {$t_{21}|t_{21}$};
  \draw [->] (0) ..controls (29.417bp,75.815bp) and (31.092bp,116.0bp)  .. (39.5bp,116.0bp) .. controls (47.054bp,116.0bp) and (49.174bp,83.563bp)  .. (0);
  \draw (9.0bp,108.5bp) node {$t_{22}|t_{22}$};
%
\end{tikzpicture}

==> backup/Automatica_submission/prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

We denote the set of natural numbers by $\nat$. For $n \in \nat$, let $[n] = \{1,..,n\}$. We denote set cardinality by $\abs{S}$, power set by $2^S$, and set subtraction by $S_1 \backslash S_2 = \set{s \in S_1}{s \notin S_2}$. We also write ``iff'' for ``if and only if''.


We follow the common notations for sequences. For a given finite set of symbols, a finite-length sequence of symbols is called a word. A set of words is called a language. A word can be viewed as a singleton language. The empty word is denoted by $\epsilon$. The concatenation of two languages (or words) is defined by
$$L_1 L_2 = \{I_1 I_2 \ \vert \ I_1 \in L_1, I_2 \in L_2\}.$$
The Kleene star (i.e., finite repetition) of a language (or word) is defined by 
$L^* = \set{I_1 \ldots I_n}{I_1, \ldots, I_n \in L, n \in \nat}$; by convention, $\varepsilon \in L^*$. 
The union of two languages (or words) is denoted by $[L_1, L_2]$. 
%
A language is \emph{regular} if it can be represented only using union, concatenation, and Kleene star~\cite{sipser_IntroductionTheoryComputation_1996}.
In addition, a word $I_1$ is a prefix of another word $I$ if there exists $I_2$ such that $I = I_1 I_2$. The prefix closure $\overline{L}$ of a language $L$ is derived by including all prefixes of all $I \in L$ in $\overline{L}$. A language $L$ is prefix-closed if $L =  \overline{L}$.


We call $\rr \subseteq  S_1 \times S_2$ a relation between two sets $S_1$ and $S_2$. With slight abuse of notation, the image of a subset $S_1' \subseteq  S_1$ (an element is viewed a singleton set) over the relation $\rr$ is defined by 
$$\rr(S_1') = \set{s_2 \in S_2 }{s_1 \in S_1', (s_1, s_2) \in \rr}.$$ The relation $\rr$ is a partial function if $\abs{\rr(s_1)} \leq 1$ for any $s_1 \in S_1$. The inverse of the relation $\rr$ is defined by 
$$\rr^{-1} = \set{(s_2, s_1)}{(s_1, s_2) \in \rr},$$ 
whereas the composition of two relations is defined by 
$$\rr_1 \circ \rr_2 = \set{(s_1, s_3)}{\exists s_2. \ (s_1, s_2) \in \rr_1, (s_2, s_3) \in \rr_2}.$$ 


\yw{\begin{definition}
\label{def:regular relation}
For two finite sets $\ainputs$ and $\aoutputs$, the relation $\rr \subseteq \ainputs^* \times \aoutputs^*$ is a regular relation iff 
$$\big\{ (\ainput_1, \aoutput_1) \ldots (\ainput_n, \aoutput_n) \mid  (\ainput_1 \ldots \ainput_n, \aoutput_1 \ldots \aoutput_n) \in \rr \big\}$$
is a regular language over $\ainputs \times \aoutputs$. Here, $\ainput_1, \aoutput_1, \ldots \ainput_n,  \aoutput_n$ can be $\varepsilon$.
\end{definition}}


Similar to the relationship between regular languages and automata, regular relations can be graphically represented by finite-state transducers.


\begin{definition}
\label{def:fst}
A finite-state transducer (FST) is a tuple $\attacker = (\astates, \ainit, \ainputs, \aoutputs, \atransitions, \allowbreak \afinal)$ where
\begin{itemize}[leftmargin=0.5cm]
  \item $\astates$ is a finite set of states;
  \item $\ainit \in \astates$ is the initial state;
  \item $\ainputs$ is a finite set of input symbols;
  \item $\aoutputs$ is a finite set of output symbols;
  \item $\atransitions \subseteq \astates \times \big( \ainputs \cup \{ \epsilon \} \big) \times \big( \aoutputs \cup \{ \epsilon \} \big) \times \astates$ is a transition relation;
  \item $\afinal \subseteq \astates$ is a finite set of final states.
\end{itemize}
\end{definition}

FSTs can be viewed as automata that have both input and output symbols on their transitions. Accordingly, automata are treated as FSTs with identical input and output. More terminology on FSTs is provided below.

\begin{itemize}[leftmargin=10pt]
  \item[-] An \emph{execution} is a sequence of transitions $(\astate_0, \ainput_1, \aoutput_1, \astate_1) \allowbreak ... (\astate_{n-1}, \ainput_n, \aoutput_n, \astate_n)$ where $\astate_0 = \ainit$ and $(\astate_{i-1}, \ainput_i, \aoutput_i, \astate_i) \allowbreak \in \atransitions$ for $i \in [n]$. 
  \item[-] The FST $\attacker$ defines a relation between $\ainputs^*$ and $\aoutputs^*$ by $\rr_\attacker = \{(\ainput_1 ... \ainput_n, \ \aoutput_1 ... \aoutput_n) \ \vert \ \exists \textrm { an execution } (\ainit, \ainput_1, \allowbreak \aoutput_1, \astate_1) ... (\astate_{n-1}, \ainput_n, \aoutput_n, \astate_n) \textrm{ and } \astate_n \in \afinal\}$. 
  \item[-] The \emph{input language} and \emph{output language} of $\attacker$ are defined by $L_{\mathrm{in}}(\attacker) = \rr_\attacker^{-1} (\aoutputs^*)$ and $L_{\mathrm{out}}(\attacker) = \rr_\attacker (\ainputs^*)$.
  % \item[-] The \emph{reachset} of the input word $I \in L_{\mathrm{in}} (\attacker)$ is $\reach_\attacker(I) = \{\astate_n \in \astates \ \vert \ \exists \textrm { an execution } (\ainit, \ainput_1, \aoutput_1, \astate_1) \allowbreak ... (\astate_{n-1}, \ainput_n, \aoutput_n, \astate_n) \textrm{ and } I = \ainput_1 ... \ainput_n\}$.
\end{itemize}

\yw{\paragraph*{Determinism of FSTs.}
There are several notions of determinism for FSTs. The FST $\attacker$ is \emph{deterministic} if at most one execution exists for a \textbf{pair} of input and output words. The FST $\attacker$ is \textit{deterministic-in-input} or \textit{deterministic-in-output} if at most one execution exists for an input or an output word, respectively. Accordingly, a deterministic FST can be nondeterministic-in-input and/or output. % \todo{can it be and?}  
}

\yw{
An FST defines a regular relation. In addition, for any regular relation, we can construct a corresponding FST~\cite{holcombe_AlgebraicAutomataTheory_1982}.
}
The expressiveness of FSTs does not change by allowing a sequence of input/output symbols on single transitions because they can be reduced to FSTs in Definition~\ref{def:fst} through normalization~\cite{holcombe_AlgebraicAutomataTheory_1982,mohri_WeightedAutomataAlgorithms_2009}. \yw{A nondeterministic FST is determinizable without changing its regular relation by the powerset construction for automata (i.e., by viewing a pair of input and output symbols as a single symbol)~\cite{sipser_IntroductionTheoryComputation_1996}. 
Thus, in this work, we focus on deterministic FSTs (but potentially non-deterministic in the more standard input/output view}. %\todo{check}




% Finally, we introduce determinism-in-input, which implies the current state of an FST can be uniquely decided only by the past input symbols.

% \begin{definition} \label{def:determinism}
% The FST in Definition~\ref{def:fst} is deterministic-in-input iff $\atransitions (\astate, \ainput, \cdot, \cdot)$ is a partial function.
% \end{definition}








==> backup/Automatica_submission/supervisor.tex <==
\begin{tikzpicture}[>=latex,line join=bevel,scale=0.42]
%%
\node (10) at (655.5bp,98.0bp) [draw,circle, double,solid] {$10$};
  \node (1) at (180.0bp,98.0bp) [draw,ellipse,solid] {$1$};
  \node (0) at (22.0bp,98.0bp) [draw,circle, double,initial,initial text=] {$0$};
  \node (3) at (180.0bp,40.0bp) [draw,circle, double,solid] {$3$};
  \node (2) at (180.0bp,156.0bp) [draw,circle, double,solid] {$2$};
  \node (5) at (338.0bp,174.0bp) [draw,circle, double,solid] {$5$};
  \node (4) at (338.0bp,98.0bp) [draw,circle, double,solid] {$4$};
  \node (7) at (496.0bp,98.0bp) [draw,ellipse,solid] {$7$};
  \node (6) at (338.0bp,22.0bp) [draw,circle, double,solid] {$6$};
  \node (9) at (496.0bp,40.0bp) [draw,circle, double,solid] {$9$};
  \node (8) at (496.0bp,156.0bp) [draw,circle, double,solid] {$8$};
  \draw [->] (0) ..controls (46.924bp,84.44bp) and (53.13bp,81.434bp)  .. (59.0bp,79.0bp) .. controls (88.792bp,66.646bp) and (124.0bp,55.689bp)  .. (3);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (101.0bp,86.5bp) node {$t_{21}|t_{21}$};
  \draw [->] (3) ..controls (204.94bp,26.676bp) and (211.07bp,24.324bp)  .. (217.0bp,23.0bp) .. controls (246.47bp,16.426bp) and (280.99bp,16.919bp)  .. (6);
  \draw (259.0bp,30.5bp) node {$t_{22}|t_{22}$};
  \draw [->] (0) ..controls (46.924bp,111.56bp) and (53.13bp,114.57bp)  .. (59.0bp,117.0bp) .. controls (88.792bp,129.35bp) and (124.0bp,140.31bp)  .. (2);
  \draw (101.0bp,152.5bp) node {$\epsilon|t_{11}$};
  \draw [->] (5) ..controls (386.9bp,168.43bp) and (432.75bp,163.21bp)  .. (8);
  \draw (417.0bp,176.5bp) node {$t_{21}|t_{21}$};
  \draw [->] (4) ..controls (363.62bp,109.5bp) and (369.5bp,111.93bp)  .. (375.0bp,114.0bp) .. controls (411.71bp,127.8bp) and (422.14bp,127.62bp)  .. (459.0bp,141.0bp) .. controls (461.25bp,141.82bp) and (463.57bp,142.69bp)  .. (8);
  \draw (417.0bp,148.5bp) node {$\epsilon|t_{12}$};
  \draw [->] (4) ..controls (388.46bp,98.0bp) and (436.92bp,98.0bp)  .. (7);
  \draw (417.0bp,110.5bp) node {$t_{22}|t_{12}$};
  \draw [->] (6) ..controls (384.68bp,17.219bp) and (425.17bp,15.453bp)  .. (459.0bp,23.0bp) .. controls (461.69bp,23.6bp) and (464.42bp,24.411bp)  .. (9);
  \draw (417.0bp,30.5bp) node {$\epsilon|t_{11}$};
  \draw [->] (7) ..controls (540.43bp,98.0bp) and (588.92bp,98.0bp)  .. (10);
  \draw (575.0bp,110.5bp) node {$\epsilon|t_{22}$};
  \draw [->] (1) ..controls (224.27bp,98.0bp) and (272.98bp,98.0bp)  .. (4);
  \draw (259.0bp,110.5bp) node {$\epsilon|t_{21}$};
  \draw [->] (8) ..controls (541.76bp,143.22bp) and (582.84bp,130.85bp)  .. (617.0bp,117.0bp) .. controls (619.72bp,115.9bp) and (622.51bp,114.68bp)  .. (10);
  \draw (575.0bp,152.5bp) node {$t_{22}|t_{22}$};
  \draw [->] (9) ..controls (541.76bp,52.775bp) and (582.84bp,65.153bp)  .. (617.0bp,79.0bp) .. controls (619.72bp,80.103bp) and (622.51bp,81.315bp)  .. (10);
  \draw (575.0bp,86.5bp) node {$\epsilon|t_{12}$};
  \draw [->] (0) ..controls (72.457bp,98.0bp) and (120.92bp,98.0bp)  .. (1);
  \draw (101.0bp,110.5bp) node {$t_{21}|t_{11}$};
  \draw [->] (2) ..controls (228.9bp,161.57bp) and (274.75bp,166.79bp)  .. (5);
  \draw (259.0bp,176.5bp) node {$\epsilon|t_{12}$};
  \draw [->] (3) ..controls (225.83bp,52.586bp) and (266.95bp,64.881bp)  .. (301.0bp,79.0bp) .. controls (303.84bp,80.179bp) and (306.77bp,81.492bp)  .. (4);
  \draw (259.0bp,86.5bp) node {$\epsilon|t_{11}$};
  \draw [->] (4) ..controls (362.92bp,84.44bp) and (369.13bp,81.434bp)  .. (375.0bp,79.0bp) .. controls (404.79bp,66.646bp) and (440.0bp,55.689bp)  .. (9);
  \draw (417.0bp,86.5bp) node {$t_{22}|t_{22}$};
  \draw [->] (2) ..controls (205.94bp,145.17bp) and (211.66bp,142.94bp)  .. (217.0bp,141.0bp) .. controls (253.86bp,127.62bp) and (264.29bp,127.8bp)  .. (301.0bp,114.0bp) .. controls (303.41bp,113.09bp) and (305.89bp,112.12bp)  .. (4);
  \draw (259.0bp,148.5bp) node {$t_{21}|t_{21}$};
%
\end{tikzpicture}

==> backup/backup.tex <==


    


Since designing a resilient supervisor is not always possible, we consider a related problem of designing a weakly-resilient supervisor that achieves the minimal super-language of the desired language $\desired$.


\begin{definition}
\label{def:weak supervisor}
The FST $\supervisor$ is a weakly-resilient supervisor for a desired language $\desired$ iff
\begin{itemize}
  \item $\desired \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a, \attacker_s)$, and
  \item for any $\supervisor'$ that satisfies 
  $\desired \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor', \attacker_a, \attacker_s)$, it holds that 
  $L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a, \attacker_s) \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor', \attacker_a, \attacker_s)$.
\end{itemize}
\end{definition}


Generally, designing weakly-resilient supervisors is possible. And designing a resilient supervisor is possible iff the weakly-resilient supervisor is resilient (see Section~\ref{sec:design} for details). 


==> bio.tex <==
% !TEX root = tac19.tex

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{yw_small.jpg}}]{Yu Wang}
% is currently a Postdoctoral Associate in the Department of Electrical and Computer Engineering at Duke University. He received his Ph.D. degree in Mechanical Engineering and his M.S. degrees in Statistics, Mathematics, and Mechanical Engineering in 2018, 2017, 2016 and 2014, respectively from the University of Illinois at Urbana-Champaign. Before that, he received his B.S. degree in Engineering Mechanics from the School of Aerospace of Tsinghua University in 2012.
% \end{IEEEbiography}


% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{alper.png}}]
% {Alper Kamil Bozkurt} received the B.S. and M.S. degrees in computer engineering from Bogazici University, Turkey, in 2015 and 2018, respectively. He is currently a Ph.D. student in the Department of Computer Science at Duke University. His research interests lie at the intersection of machine learning, control theory, and formal methods. In particular, he focuses on developing learning based algorithms that synthesize provably safe and reliable controllers for cyber-physical systems.


% \end{IEEEbiography}



% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pajic.jpg}}]{Miroslav Pajic}
%  (S'06-M'13-SM'19) received the Dipl. Ing. and M.S. degrees in electrical engineering from the University of Belgrade, Serbia, in 2003 and 2007, respectively, and the M.S. and Ph.D. degrees in electrical engineering from the University of Pennsylvania, Philadelphia, in 2010 and 2012, respectively.

% He is currently the Nortel Networks Assistant Professor in the Department of Electrical and Computer Engineering at Duke University. He also holds a secondary appointment in the Computer Science Department. His research interests focus on the design and analysis of cyber-physical systems, and in particular security-aware distributed/networked control systems, embedded systems, and high-confidence control systems.

% Dr. Pajic received various awards including the ACM SIGBED Early-Career Award, IEEE TCCPS Early-Career Award, NSF CAREER Award, ONR Young Investigator Program Award, ACM SIGBED Frank Anger Memorial Award, Joseph and Rosaline Wolf Best Dissertation Award from Penn Engineering, IBM Faculty Award, as well as six Best Paper and Runner-up Awards, such as the Best Paper Awards at the 2017 ACM SIGBED International Conference on Embedded Software (EMSOFT) and 2014 ACM/IEEE International Conference on Cyber-Physical Systems (ICCPS), and the Best Student Paper award at the 2012 IEEE Real-Time and Embedded Technology and Applications Symposium (RTAS). He is an associate editor in the ACM Transactions on Computing for Healthcare (ACM HEALTH) and a co-chair of the 2019 ACM/IEEE International Conference on Cyber-Physical Systems~(ICCPS'19).

% \end{IEEEbiography}


==> input_attack.tex <==
\subsection{Supervisor Design Resilient to Actuator Attacks}
\label{sub:actuator attacks}

Unlike sensor attacks, {designing FST-based supervisors that are resilient to actuator attacks is not always possible (even if they can revise undesirable symbols).
% when FSTs are used to capture the supervisor's functionality.
}
% \todo{check} 
For example, if no actuation symbols are updated (i.e., the attacker $\attacker_a$ blocks all symbols from the supervisor $\plant$ in the control loop of Fig.~\ref{fig:control}), designing a resilient supervisor is impossible for any desired language $\desired$ (except for $\desired = \{\epsilon\}$). In this example, the infeasibility of resilient supervisors is caused by the restriction of the output language $L_{\mathrm{out}} (\attacker_a)$; to rule out this trivial case, we make the following technical assumption (otherwise, we can consider $\desired \cap L_{\mathrm{out}} (\attacker_a)$ instead of $\desired$).

\begin{assumption}
The output language of the attacks $\attacker_a$, in Fig.~\ref{fig:control}, contains the desired language $\desired$, i.e., $\desired \subseteq L_{\mathrm{out}} (\attacker_a)$.
\end{assumption}

Even under the above assumption, designing a resilient supervisor may still be unfeasible. 
Below, we present the condition for the design of attack-resilient supervisors for actuator attacks.

\begin{theorem}
\label{prop:actuator attack}
Without sensor attacks (in Fig.~\ref{fig:control}), for any plant $\plant$ and desired (prefix-closed regular) language $\desired \subseteq L_{\mathrm{in}}(\plant)$, the FST 
$$\supervisor = \plant^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1}$$
is a candidate resilient supervisor (to the actuator attack $\attacker_a$) with
$$L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a) = \rr_{\attacker_a^{-1} \c \attacker_a} (\desired).$$
Particularly, $\supervisor$ is a resilient supervisor iff 
% \todo{just if? not iff?}
$$\rr_{\attacker_a^{-1} \c \attacker_a} (\desired) = \desired.$$
\end{theorem}


\begin{proof}
We defer the proof until Theorem 3.
% It suffices to show the language sent to the plant is exactly $\rr_{\attacker_a^{-1} \c \attacker_a} (\desired)$ under the supervisor $\supervisor = \plant^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1}$. Since 
% $$L_{\mathrm{out}} (\supervisor \c \attacker_a) \subseteq L_{\mathrm{out}} (\mathcal{M}_\desired \c {\attacker_a^{-1}} \c {\attacker_a}) \subseteq \rr_{\attacker_a^{-1} \c \attacker_a} (\desired),$$ 
% the plant only receives words in $\rr_{\attacker_a^{-1} \c \attacker_a} (\desired)$. On the other hand, for any $I \in \rr_{\attacker_a^{-1} \c \attacker_a} (\desired)$, from Lemma~\ref{lem:id} it holds that
% \yw{\[
% \begin{split}
% & I \in \rr_{\attacker_a^{-1} \c \attacker_a} (I) \subseteq \rr_{\plant \c \plant^{-1}} \c \rr_{\mathcal{M}_\desired} \c \rr_{\attacker_a^{-1} \c \attacker_a} (I)
% \\ & \quad = \rr_{\plant \c \plant^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1} \c \attacker_a} (I) = \rr_{\plant \c \supervisor \c \attacker_a} (I).
% \end{split}
% \]}
% Thus, the word $I$ can be sent to the plant.
% We now show the minimality of $L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a)$. Suppose there is another weakly-resilient supervisor $\supervisor'$ such that
% \begin{equation} \label{eq:pf_1}
%   \desired \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor', \attacker_a)  \subseteq L_{\mathrm{in}}(\plant \ \vert \ \supervisor, \attacker_a).
% \end{equation}
% For simplicity, let $L' = L_{\mathrm{in}}(\plant \ \vert \ \supervisor', \attacker_a)$.
% For any input word $I' \in L'$ of the plant, there exists an output word $I$ of the supervisor such that $I \in \rr_{\attacker_a^{-1}} (I')$.
% For the word $I$, any revision by the attacker $\attacker_a$ can possibly be sent to the plant, so we have $\rr_{\attacker_a} (I) \subseteq L'$. Therefore, we have
% \begin{equation} \label{eq:pf_2}
%   \rr_{\attacker_a^{-1} \c {\attacker_a}} (L') \subseteq L'
% \end{equation}
% Combining \eqref{eq:pf_1} and \eqref{eq:pf_2}, we have $L' = \rr_{\attacker_a^{-1} \c \attacker_a} (\desired)$ since
% $\rr_{\attacker_a^{-1} \c {\attacker_a}} (\desired) \subseteq \rr_{\attacker_a^{-1} \c {\attacker_a}} (L') \subseteq L'$. 
\end{proof}




Intuitively, in the supervisor $\supervisor = \plant^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1}$, the part $\plant^{-1}$ partially recovers the plant's input from the output, then the part $\mathcal{M}_\desired$ filters out undesirable words, and finally the part $\attacker_a^{-1}$ prepares (not perfectly) for the attacks of $\attacker_a$. Theorem~\ref{prop:actuator attack} also directly leads to a  method for design of  supervisors resilient to actuator attacks, summarized in Algorithm~\ref{alg:actuator attack}.







\begin{algorithm}[!t]
\caption{Resilient supervisor for actuator attacks}
\label{alg:actuator attack}
\begin{algorithmic}[1]
\Require{Plant $\plant$, desired language $\desired \subseteq L_{\mathrm{in}}(\plant)$, and actuator attacker $\attacker_a$.}
\State{Build an automaton $\mathcal{M}_\desired$ for $\desired$.}
\State{Compute the inverse $\attacker_a^{-1}$ and $\plant^{-1}$.}
\State{Compute serial composition $\supervisor =  \plant^{-1} \c \mathcal{M}_\desired \c \attacker_a^{-1}$.}
\If{$\rr_{\attacker_a^{-1} \c \attacker_a} (\desired) = \desired$}
\State \Return $\supervisor$
\Else
\State \Return Infeasible
\EndIf
\end{algorithmic}
\end{algorithm}







\begin{example}
\label{ex:input_attack}
Without sensor attacks (in Fig.~\ref{fig:control}), consider:
% \begin{itemize}
%   \item 
  a set of symbols $\ainputs = \{\ainput_1,\ainput_2\}$;
%   \item 
  a plant $\plant$ with input language $[\ainput_1, \ainput_2]^*$ as shown in Fig.~\ref{fig:input_plant}; and
%   \item 
  a desired language $\desired = \overline{[\ainput_1, \ainput_2] \ainput_2}$ modeled by automaton $\mathcal{M}_\desired$ in Fig.~\ref{fig:input_desired}.
% \end{itemize}
%
For the actuator attacks $\attacker_a$ from Fig.~\ref{fig:input_attack_1} that rewrite the first $\ainput_1$ nondeterministically to $\ainput_1$ or $\ainput_2$, the supervisor in Fig.~\ref{fig:input_supervisor_1} derived by Algorithm~\ref{alg:actuator attack} is resilient. 

For the actuator attacks $\attacker_a$ from Fig.~\ref{fig:input_attack_2} that rewrite any $\ainput_1$ nondeterministically to $\ainput_1$ or $\ainput_2$, Algorithm~\ref{alg:actuator attack} gives a candidate resilient supervisor shown in Fig.~\ref{fig:input_supervisor_1}, and the minimal super-language is $\overline{[\ainput_1, \ainput_2] [\ainput_1, \ainput_2]}$. The supervisor cannot achieve exactly the desired language $\overline{[\ainput_1, \ainput_2] \ainput_2}$ which requires the second symbol to be $\ainput_2$ because the attacker $\attacker_a$ can always rewrite it to $\ainput_1$. 
\end{example}

\begin{figure}
\centering
\subcaptionbox{Plant.\label{fig:input_plant}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (s) {$0$};
  \path[->] (s) edge[loop right] node {\begin{minipage}{12pt}$\ainput_1 \vert \ainput_1$\\$\ainput_2 \vert \ainput_2$\end{minipage}} ();
\end{tikzpicture}
}
\subcaptionbox{Automaton of $\desired$.\label{fig:input_desired}}[.5\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0] (1) {$1$};
  \node[state,right of=1] (2) {$2$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1$} (1)
  (0) edge[bend right] node[below] {$\ainput_2$} (1)
  (1) edge[bend left] node[above] {$\ainput_2$} (2);

  % \path[->] (0) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1$} (1)
  % (0) edge[bend right] node[below] {$\ainput_2 \vert \ainput_2$} (1)
  % (1) edge[bend left] node[above] {$\ainput_1 \vert \epsilon$} (2)
  % (1) edge[bend right] node[below] {$\ainput_2 \vert \ainput_2$} (2)
  % (2) edge[loop right] node[right] {$\ainput_1, \ainput_2 \vert \epsilon$} (2);
\end{tikzpicture}
}


\par\bigskip
\subcaptionbox{Actuator Attacker I.\label{fig:input_attack_1}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0] (1) {$1$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1$} (1)
  (0) edge[bend right] node[below] {$\ainput_1 \vert \ainput_2$} (1)
  (1) edge[loop right] node[right] {\begin{minipage}{0pt}$\ainput_1 \vert \ainput_1$\\$\ainput_2 \vert \ainput_2$\end{minipage}} (1);
\end{tikzpicture}
}
\hspace{0.2cm}
\subcaptionbox{Supervisor I.\label{fig:input_supervisor_1}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0] (1) {$1$};
  \node[state,right of=1] (2) {$2$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1$} (1)
  (0) edge[bend right] node[below] {$\ainput_2 \vert \ainput_1$} (1)
  (1) edge[bend left] node[above] {$\ainput_2 \vert \ainput_2$} (2);
\end{tikzpicture}
}


\par\bigskip
\subcaptionbox{Actuator Attacker II.\label{fig:input_attack_2}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \path[->] (0) edge[loop above] node {$\ainput_1, \ainput_2 \vert \ainput_1, \ainput_2$} (0);
\end{tikzpicture}
}
\subcaptionbox{Supervisor II.\label{fig:input_supervisor_2}}[.5\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0,xshift=0.3cm] (1) {$1$};
  \node[state,right of=1,xshift=0.3cm] (2) {$2$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1, \ainput_2$} (1)
  (0) edge[bend right] node[below] {$\ainput_2 \vert \ainput_1, \ainput_2$} (1)
  (1) edge[bend left] node[above] {$\ainput_2 \vert \ainput_1, \ainput_2$} (2);
  % (1) edge[bend right] node[below] {$\ainput_2 \vert \ainput_1, \ainput_2$} (2);
\end{tikzpicture}
}
\caption{Example supervisors for actuator attacks.\label{fig:input_example}}
\end{figure}





==> nondeterminism.tex <==
\subsection*{Implementability of FSTs}
Our framework allows nondeterministic FST to model the supervisor. Due to the nondeterminism, an acceptable pair input/output word is not always executable if sent symbol-by-symbol to the FST. For example, the FST in 
Fig.~\ref{fig:non_imp} allows input $\ainput_1 \ainput_2$ and output $\ainput_2 \ainput_3$ through following the state transitions $0 \to 1 \to 3$. However, if the FST first receives the input symbol $\ainput_1$ and output symbol $\ainput_2$ and then jumps to the state $2$, then the rest of the input and output symbols are not executable any more.


For example, the FST in Fig.~\ref{fig:non_imp} is non-implementable; when executing the word $\ainput_1 \ainput_2$ symbol-by-symbol, if it transits from the state $0$ to the state $2$ upon receiving the first symbol $\ainput_1$, then next symbol $\ainput_2$ will be blocked. This is captured as follows.

\begin{figure}[!t]
\centering
\subcaptionbox{Non-implementable FST.\label{fig:non_imp}}[.5\linewidth]{
\begin{tikzpicture}
	\node[state,initial, initial text=] (0) {$0$};
	\node[state,right of=0, xshift=0.4cm, yshift=0.5cm] (1) {$1$};
	\node[state,right of=0, xshift=0.4cm, yshift=-0.5cm] (2) {$2$};
	\node[state,right of=0, xshift=2cm] (3) {$3$};
	\path[->] (0) edge node[above] {$\ainput_1 \vert \ainput_2$} (1);
	\path[->] (0) edge node[below] {$\ainput_1 \vert \ainput_2$} (2);
	\path[->] (1) edge node[above] {$\ainput_2 \vert \ainput_3$} (3);
	\path[->] (2) edge node[below] {$\ainput_3 \vert \ainput_3$} (3);
\end{tikzpicture}
}
\subcaptionbox{Determinization.\label{fig:determinization}}[.48\linewidth]{
\begin{tikzpicture}
\node[state, initial, initial text=] (0) {$0$};
\node[state, right of=0, xshift=0.2cm] (1) {$1,2$};
\node[state, right of=1, xshift=0.2cm] (2) {$3$};
\path[->] (0) edge node[above] {$\ainput_1 \vert \ainput_2$} (1);            
\path[->] (1) edge[bend left] node[above] {$\ainput_2 \vert \ainput_3$} (2);                 
\path[->] (1) edge[bend right] node[below] {$\ainput_3 \vert \ainput_3$} (2);
\end{tikzpicture}
}
\caption{Examples of checking FST implementability.}
\end{figure}




\begin{definition}
\label{def:implementable}
An FST $\attacker = (\astates, \ainit, \allowbreak \ainputs, \aoutputs, \atransitions, \afinal)$ is implementable iff
\begin{align*}
& \forall I \in L_{\mathrm{in}} (\attacker) \ \forall i \in \ainputs.
\Big( \exists \astate \in \reach_\attacker (I). \ \atransitions(\astate, \ainput, \cdot, \cdot)  
\\ & \neq \emptyset \Big) \implies
\Big( \forall \astate \in \reach_\attacker (I). \ \atransitions(\astate, \ainput, \cdot, \cdot) \neq \emptyset \Big)  
\end{align*}
where $\reach_\attacker (I)$ is the reachset of the {input} word 
% \todo{Check} 
$I$. 
\end{definition}

Definition~\ref{def:implementable} means that if an input symbol is enabled on a state of $\astate \in \reach_\attacker (I)$ then it should be also enabled on all states of $\astate \in \reach_\attacker (I)$. It ensures that every enabled symbol can be executed regardless of the FST's past (nondeterministic) executions. For deterministic FSTs, $\abs{\reach_\attacker (I)}=1$ for any $I \in L_{\mathrm{in}} (\attacker)$, and thus the following lemma directly holds.
% \todo{check}

\begin{lemma}
Deterministic FSTs are implementable.
\end{lemma}

Checking implementability directly by Definition~\ref{def:implementable} is impractical, as it requires evaluating the above condition for all $I \in L_{\mathrm{in}} (\attacker)$. To resolve this issue, we introduce the input-determinization for FSTs based on the powerset construction for automata~\cite{sipser_IntroductionTheoryComputation_1996}.

\begin{definition}
The input-determinization of the FST $\attacker = (\astates, \ainit, \ainputs, \aoutputs, \atransitions, \afinal \allowbreak = \astates)$ 
is an automata $\attacker^D = (\astates^D, \ainit^D, \ainputs^D, \atransitions^D, \afinal^D = \astates^D)$ constructed as:  
\begin{itemize}[leftmargin=10pt]
\item[-] Let $\astates^D = 2^\astates$, $\ainit^D = \{\ainit\}$, and $\ainputs^D = \ainputs$.
\item[-] Let $(\astates_1, \ainput, \astates_2) \in \atransitions^D$ iff
\begin{itemize}
\item $\astates_1 \subseteq \astates$ and $\ainput \in \ainputs$, 
\item $\astate \in \astates_2$ iff there exists a sequence $(\astate_0, \ainput_1, \aoutput_1, \astate_1) \allowbreak ... (\astate_{n-1}, \ainput_n, \aoutput_n, \astate_n)$ with
$s_0 \in S_1$,
$s_n = s$, and
$(\astate_{i-1}, \ainput_i, \aoutput_i, \astate_i) \in \atransitions$ for $i \in [n]$ such that
$\ainput_1 ... \ainput_n = \ainput$ (i.e., one of $\ainput_1, ..., \ainput_n$ is $\ainput$ and all
% \todo{check}  
others are $\varepsilon$).
\end{itemize}
\item[-] Remove unreachable states (from $\ainit^D$) in $\astates^D$.
\end{itemize}
\end{definition}


The states of $\attacker^D$ are the powerset of the states of $\attacker$. Both $\attacker$ and $\attacker^D$ take input symbols from $\ainputs$. A transition $(\astates_1, \ainput, \astates_2)$ exists in $\astates^D$ iff $\astates_2$ is exactly those states in $\attacker$ that can be reached from some state in $\astates_1$ by taking an input symbol $\ainput$ (maybe through multiple transition as there are transitions with $\varepsilon$ input). 


Following the same approach as in~\cite{sipser_IntroductionTheoryComputation_1996}, it holds that the automata $\attacker^D$ is deterministic and free from $\varepsilon$-moves. Besides, $\attacker^D$ defines the same regular relation as $\attacker$. 
Furthermore, due to the determinism of $\attacker^D$, for any input word $I$, the reachset $\reach_{\attacker^D} (I)$ is a singleton and equal to  
$\{\reach_\attacker(I)\}$.
Since we have removed unreachable states in $\attacker^D$, when $I$ runs over $L_{\mathrm{in}} (\attacker)$, $\reach_\attacker(I)$ runs over all the states of $\attacker^D$. Thus, the following lemma holds.


\begin{lemma} \label{lem:check_implementable}
The {FST} $\attacker$
% \todo{why the plant?} 
is implementable iff
\begin{align*}
& \forall \astate^D \in \astates^D \ \forall i \in \ainputs.
\Big( \exists \astate \in \astate^D. \ \atransitions(\astate, \ainput, \cdot, \cdot)  
\\ & \neq \emptyset \Big) \implies
\Big( \forall \astate \in \astate^D. \ \atransitions(\astate, \ainput, \cdot, \cdot) \neq \emptyset \Big)  
\end{align*}
\end{lemma}

Lemma~\ref{lem:check_implementable} can be directly used to check implementability by enumerating over all $\astate^D \in \astates^D$, $i \in \ainputs$ and $\astate \in \astate^D$. %Below is an example.

\begin{example}
The automaton in Fig.~\ref{fig:determinization} is the input-determinization of the FST in Figure~\ref{fig:non_imp}. The two FST states $1$ and $2$ correspond to the same automaton state $1,2$, because they are both reachable for the input $\ainput_1$. The FST is not implementable because $i_2$ is enabled on its state $1$ but not state $2$.   
\end{example}


% \begin{assumption} \label{ass:implementable}
% In the rest of this paper, we focus on implementable FSTs.
% \todo{is this a limitation? if no, why? if yes, how we'll address it?}
% \end{assumption}

==> output_attack.tex <==
\subsection{Supervisor Design Resilient to Sensor Attacks}
\label{sub:sensor attacks}

The presence of attacks on system sensors introduces a significant challenge for automaton-based supervisors in classical supervisory control~\cite{cassandras_IntroductionDiscreteEvent_2008}, which can only allow/disable symbols. 

In the general case, an FST-based supervisor could also insert/replace symbols, which facilitates handling sensor attacks. Even if there is no observation at all (i.e., the attacker $\attacker_s$ blocks all symbols from the plant $\plant$ in the control loop of Figure~\ref{fig:control}), we can still construct an FST-based supervisor from the automata model of the desired language $\desired$ by relabeling the transitions from $\ainput$ to $\varepsilon \vert \ainput$. When there is no actuator attack, this supervisor can restrict the plant's input words to $\desired$ without any observation from the plant. {On the other hand, if the FST-based supervisor does not insert/replace symbols, then our result reduces to classical supervisory control.}

% \todo{cehck the paragrpah}
% \todo{our results also cover when we don't allow 'generating' symbols -- add this}


The following example shows a simple regular-rewriting sensor attack that can only be handled by FST-based supervisors. It motivates the need to use FST-based supervisors instead of automaton-based supervisors.

\begin{example}
\label{ex:counter_output}
We consider the case without actuator attacks in Fig.~\ref{fig:control} and: 
%   \item 
  a set of symbols $\ainputs = \{\ainput_1, \ainput_2\}$;
%   \item 
  a plant $\plant$ with input language $[\ainput_1, \ainput_2]^*$ as shown in Fig.~\ref{fig:output_plant};
%   \item 
  a desired language $\desired = \overline{(\ainput_1 \ainput_2)^*}$ modeled by automaton $\mathcal{M}_\desired$ in Figure~\ref{fig:output_desired_1}; and
%   \item 
  sensor attacks $\attacker_s$ can be modeled by the FST in Fig.~\ref{fig:output_attack_1}. 
% \end{itemize}
Designing an automaton-based supervisor without the ability to revise symbols is impossible in this case. The reason is that the output of the supervisor should be the desired language $[\ainput_1, \ainput_2]^*$, but the input is always $\ainput_1^*$, as the plant only generates $\ainput_2^*$ and the attacker rewrites it to $\ainput_1^*$. On the other hand, there exists an FST-based resilient supervisor, shown in Fig.~\ref{fig:output_supervisor_1}. It counters the attacks by revising $\ainput_1$ back to $\ainput_2$ every other~step.
\end{example}

\begin{figure}
\centering
\subcaptionbox{Plant $\plant$\label{fig:output_plant}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state, initial, initial text=] (s) {$0$};
  \path[->] (s) edge[loop above] node {$\ainput_1,\ainput_2 \vert \ainput_2$} ();
\end{tikzpicture}
}
\subcaptionbox{Attacker $\attacker_s$\label{fig:output_attack_1}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \path (0) edge[loop above] node {$\ainput_2 \vert \ainput_1$} (0);
\end{tikzpicture}
}
\subcaptionbox{Automaton of $\desired$%
\label{fig:output_desired_1}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0] (1) {$1$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1$} (1)
  (1) edge[bend left] node[below] {$\ainput_2$} (0);
\end{tikzpicture}
}
\subcaptionbox{Supervisor $\supervisor$\label{fig:output_supervisor_1}}[.45\linewidth]{
\begin{tikzpicture}
  \node[state,initial, initial text=] (0) {$0$};
  \node[state,right of=0] (1) {$1$};
  \path[->] (0) edge[bend left] node[above] {$\ainput_1 \vert \ainput_1$} (1)
  (1) edge[bend left] node[below] {$\ainput_1 \vert \ainput_2$} (0);
\end{tikzpicture}
}
\caption{Example supervisor for sensor attacks.\label{fig:output_example}}
\end{figure}
  

As illustrated in Example~\ref{ex:counter_output}, the supervisor needs the ability to recover the symbols that are revised by the FST-based sensor attacks. This naturally connects to the inversion operation of FSTs. 

\paragraph*{Inversion} The inversion of an FST is derived by flipping the input/output symbols on each transition, as given in Algorithm~\ref{alg:inversion}. Since FSTs define regular relations, Algorithm~\ref{alg:inversion} also provides an FST realization for the inversion of regular relations.

\begin{lemma}[\cite{holcombe_AlgebraicAutomataTheory_1982}]
\label{lem:inversion}
For an FST $\attacker$,
%\todo{doesn't make sense -- 2 FST? only A used?} 
it holds that $\rr_{\attacker^{-1}} = \rr_{\attacker}^{-1}$,
where $\rr_\attacker$ denotes the regular relation defined by $\attacker$.
\end{lemma}

\begin{algorithm} [!t]
\caption{FST Inversion}
\label{alg:inversion}
\begin{algorithmic}[1]
\Require{FST $\attacker = (\astates, \ainit, \ainputs, \aoutputs, \atransitions, \afinal)$}

\State{Let $\attacker^{-1} = (\astates, \ainit, \aoutputs, \ainputs, \emptyset, \afinal)$.}

\For{$(\astate, I, O, \astate') \in \atransitions$}

\State{Add transition $(\astate, O, I, \astate')$ to $\attacker^{-1}$.}

\EndFor

\State \Return{$\attacker^{-1}$}
\end{algorithmic}
\end{algorithm}



From Algorithm~\ref{alg:inversion} and Lemma~\ref{lem:inversion}, the following statements on the FST inversion easily hold.

\begin{lemma}
\label{lem:id}
For any FST $\attacker$, it holds that 
\begin{align*}
& \forall I \in L_{\mathrm{in}}(\attacker). \ I \in \rr_{\attacker \c \attacker^{-1}} (I),   
\\ & \forall I \in L_{\mathrm{out}}(\attacker). \ I \in \rr_{\attacker^{-1} \c \attacker} (I).
\end{align*}
Equivalently, it holds that
\[
\rr_{\mathcal{M}_{L_{\mathrm{in}}(\attacker)}} \subseteq \rr_{\attacker \c \attacker^{-1}}, \quad \rr_{\mathcal{M}_{L_{\mathrm{out}}(\attacker)}} \subseteq \rr_{\attacker^{-1} \c \attacker},
\]
where $L_{\mathrm{in}}$ and $L_{\mathrm{out}}$ is the input and output language of an FST and $\mathcal{M}$ stands for an automaton (thus also an FST) of a regular language. 
\end{lemma}

{For general $I \in L_{\mathrm{in}}(\attacker)$ (and similarly for $I \in L_{\mathrm{out}}(\attacker)$), we have $\{I\} \neq \rr_{\attacker \c \attacker^{-1}} (I)$, i.e., the inversion $\attacker^{-1}$ can only partially revert the effect of $\attacker$, due to the nondeterminism in input of $\attacker$. However, we can still use FST inversion to design supervisors resilient to the sensor attacks, as shown below.}
% \todo{add something like "specifically, the supervisor would provide....} 


\begin{theorem}
\label{prop:sensor attack}
Without actuator attacks (in Fig.~\ref{fig:control}), for any plant $\plant$ and desired (prefix-closed regular) language $\desired \subseteq L_{\mathrm{in}}(\plant)$, the FST $$\supervisor = \attacker_s^{-1} \c \plant^{-1} \c \mathcal{M}_\desired$$ is a resilient supervisor for the sensor attack $\attacker_s$.%
\footnote{In the following, we assume the derived $\supervisor$ is deterministic. Otherwise, we can determinize it as discussed in Section~\ref{sec:prelim}.}
\end{theorem}

\begin{proof}
It suffices to show the language passing the plant is exactly $\desired$ under the supervisor $\supervisor = \attacker_s^{-1} \c \plant^{-1} \c \mathcal{M}_\desired$.
%
By construction, the supervisor only generates words contained in $\desired$.
%
On the other hand, by Lemma~\ref{lem:id}, for any $I \in \desired$, it holds that $I \in \rr_{(\plant \c \attacker_s) \c (\plant \c \attacker_s)^{-1}} (I)$. Thus, we have $I \in \rr_{\plant \c \attacker_s \c \supervisor} (I)$, namely, the word $I$ is allowed to transmit to the plant.
\end{proof}


Intuitively, in the supervisor $\supervisor = \attacker_s^{-1} \c \plant^{-1} \c \mathcal{M}_\desired$, the part $\attacker_s^{-1}$ partially reverts the attacks of $\attacker_s$, then the part $\plant^{-1}$ partially recovers the plant's input, and finally the part $\mathcal{M}_\desired$ filters out undesirable words. Theorem~\ref{prop:sensor attack} leads to a design method for resilient supervisors to sensor attacks in Algorithm~\ref{alg:sensor attack}. 

\begin{example}
{
Following Example~\ref{ex:counter_output}, we can use Algorithm~\ref{alg:sensor attack} to derive the resilient supervisor $\supervisor$ in Fig.~\ref{fig:output_supervisor_1}. The FST $\supervisor$ can revise the symbol $\ainput_1$ to $\ainput_2$. This ability to revision is necessary to achieve attack-resilience against this attack; if we disallow symbol revision and only consider classical automata-based supervisors, then designing a resilient supervisor is impossible for these attacks, because the desired language contains $\ainput_2$ but the supervisor only receives $\ainput_1$.
}
\end{example}
% \todo{again, here it is critical to have discussion on what are our results when we have to use automaton -- this is a classical DES view}

  
  

\begin{algorithm}[!t]
\caption{Resilient supervisor for sensor attacks}
\label{alg:sensor attack}
\begin{algorithmic}[1]
\Require{Plant $\plant$, desired language $\desired \subseteq L_{\mathrm{in}}(\plant)$, and sensor attacker $\attacker_s$.}
\State{Build an automaton $\mathcal{M}_\desired$ for $\desired$.}
\State{Compute composition $\plant \c \attacker_s$.}
\State{Compute inversion $(\plant \c \attacker_s)^{-1}$.}
\State{Compute composition $\supervisor = (\plant \c \attacker_s)^{-1} \c \mathcal{M}_\desired$.}
\State \Return $\supervisor$
\end{algorithmic}
\end{algorithm}









